Specifying Non-Markovian Rewards in MDPs Using LDL on Finite Traces (Preliminary Version)

In Markov Decision Processes (MDPs), the reward obtained in a state depends on the properties of the last state and action. This state dependency makes it difficult to reward more interesting long-term behaviors, such as always closing a door after it has been opened, or providing coffee only following a request. Extending MDPs to handle such non-Markovian reward function was the subject of two previous lines of work, both using variants of LTL to specify the reward function and then compiling the new model back into a Markovian model. Building upon recent progress in the theories of temporal logics over finite traces, we adopt LDLf for specifying non-Markovian rewards and provide an elegant automata construction for building a Markovian model, which extends that of previous work and offers strong minimality and compositionality guarantees.

==> 2-ltl-finite.tex <==
\clearpage
\section{\LTLf}\label{sec:ltl-finite}

\LTLf \cite{DegVa13} uses the same syntax of the
original \LTLi \cite{Pnueli77}.\footnote{For simplicity we focus on \LTLf, however all result reported here hold aslo for its extension \LDLf, which captures \MSO on finite traces.\cite{DegVa13}.} \emph{Formulas} of \LTLf are built from a set 
$\Prop$ of propositional symbols and are closed under the boolean 
connectives, the unary temporal operator $\Next$ (\emph{next-time}) and 
the binary temporal operator $\Until$ (\emph{until}):
%%
\[\varphi ::= a \mid \lnot \varphi \mid \varphi_1\land
\varphi_2 \mid \Next\varphi \mid \varphi_1\Until\varphi_2 \text{~~~with $a\in\Prop$}\]
%%
Intuitively, $\Next\varphi$ says that $\varphi$ holds at the
\emph{next} instant, $\varphi_1\Until\varphi_2$ says that at some
future instant $\varphi_2$ will hold and \emph{until} that point
$\varphi_1$ holds.  Common abbreviations, such as $\true$, $\false$,
  $\lor$, and $\limp$ are used, including the
ones listed below:
\begin{compactitem}
\item $\Wnext\varphi = \lnot\Next\lnot\varphi$ is interpreted as a \emph{weak next}, stating that if $\Last$ does not hold then $\varphi$ must hold in the next state.
\item $\Diamond\varphi = \true\Until\varphi$
  says that $\varphi$ will \emph{eventually} hold before the last instant (included).
\item $\Box\varphi = \lnot\Diamond\lnot\varphi$
  says that from the current instant till the last instant $\varphi$ will \emph{always}
  hold.
% \item $\varphi_1 \Release \varphi_2 = \lnot(\lnot\varphi_1 \Until
%   \lnot\varphi_2)$ means that $\varphi_1$ \emph{releases} $\varphi_2$,
%   i.e., either $\varphi_2$ must hold forever, or until $\varphi_1$ also holds.
% \item $\varphi_1 \Wuntil \varphi_2 = (\varphi_1 \Until \varphi_2 \lor
%   \Box \varphi_1)$ is interpreted as a \emph{weak until}, and means that $\varphi_1$ holds until $\varphi_2$ or forever. %Notice that $\varphi_1 \Release \varphi_2$ can be also expressed as $\varphi_2 \Wuntil (\varphi_1\land\varphi_2)$.
% \item $\Last = \lnot\Next\true$ denotes the
%   last instant of the sequence. Over infinite traces it corresponds to
%   $\Next\false$ and is indeed always false, while in \LTLf it becomes
%   true at the last instance of the sequence.
% In fact wlog we assume $\Last$ to be an atomic proposition in $\Prop$
\end{compactitem}
%%
The semantics of \LTLf is given in terms of \emph{finite traces} denoting a
finite sequence of consecutive instants of time, i.e., finite words
$\pi$ over the alphabet of $2^\Prop$, containing all possible 
%propositional
 interpretations of the propositional symbols in $\Prop$. 
%%
%We use the following notation:
% \begin{itemize}
% \item Length: we denote the \emph{length} of a trace $\pi$ as $\length(\pi)$.
% \item Positions: we denote the \emph{positions}, i.e. instants, on the trace
%   as $\pi(i)$ with $0\leq i \leq \last$, where
%   $last=\length(\pi)-1$ is the last element of the trace. 
%   %We also use the notation $\pi,i$ for $\pi(i)$.
% \item Segments: we denote by $\pi(i,j)$ the \emph{segment} (i.e., the subword) obtained from
%   $\pi$ starting from position $i$ and terminating in positon $j$,
%   $0\leq i\leq j \leq \last$.
% \end{itemize}
%%
%%%%We denote the \emph{length} of a trace $\pi$ as $\length(\pi)$.
%%
%%%%We denote the \emph{positions}, i.e. instants, on the trace
%%%%  as $\pi(i)$ with $0\leq i \leq \last$, where
%%%%  $last=\length(\pi)-1$ is the last element of the trace. 
  %We also use the notation $\pi,i$ for $\pi(i)$.
%%
%%
%%GGG non credo che la usiamo
% We denote by $\pi(i,j)$ the \emph{segment} (i.e., the subword) obtained from
%   $\pi$ starting from position $i$ and terminating in positon $j$,
%   $0\leq i\leq j \leq \last$.
%%
Given a finite trace $\pi$, we inductively define when an 
\LTLf formula $\varphi$ \emph{is true} at an instant $i$  
(for $0\leq i\leq \last$), written $\pi,i\models\varphi$, as:
\begin{compactitem} 
\item $\pi,i\models a$, for $a\in\Prop$ ~iff~ $a\in\pi(i)$.
\item $\pi,i\models \lnot\varphi$ ~iff~  $\pi,i\not\models\varphi$.
\item $\pi,i\models \varphi_1\land\varphi_2$ ~iff~ $\pi,i\models\varphi_1$ and
  $\pi,i\models\varphi_2$.
\item $\pi,i\models \Next\varphi$ ~iff~ $i<\last$ and $\pi,i{+}1\models\varphi$.
\item $\pi,i\models \varphi_1\Until\varphi_2$ ~iff~ for some $j$ s.t.\ $i\leq j \leq \last$, we have
  $\pi,j\models\varphi_2$, and for all $k$, $i\leq k<j$, we have 
  $\pi,k\models\varphi_1$.
\end{compactitem}
%
A formula $\varphi$
\emph{is true} in $\pi$, in notation $\pi\models\varphi$, if
$\pi,0\models\varphi$.  
%%
% A formula $\varphi$ is \emph{satisfiable} if
% it is true in some finite trace, and it is \emph{valid} if it is true
% in every finite trace. A formula $\varphi$ logically implies a
% formula $\varphi'$, written $\varphi \models \varphi'$, if for every
% finite trace $\pi$ we have that $\pi\models\varphi$ implies
% $\pi\models\varphi'$. Notice that satisfiability, validity and
% logical implication are all mutually reducible to each other: for example 
% $\varphi$ is valid iff $\lnot\varphi$ is unsatisfiable. Similarly, $\varphi \models \varphi'$ iff
% $\varphi \land\lnot\varphi'$ is unsatisfiable.

% \begin{theorem}{\rm \cite{DegVa13}}\label{thm-LTL-PSPACE}
% Satisfiability (hence validity and logical implication) for \LTLf formulas
% is PSPACE-complete.
% \end{theorem}

Let us look at some examples.
\begin{itemize}
\item ``Safety'': $\Box\varphi$ means that always \emph{till the end of
    the trace} $\varphi$ holds.

\item ``Liveness'': $\Diamond\varphi$ means that eventually
  \emph{before the end of the trace} $\varphi$ holds. By the way, the
  term ``liveness'' is not fully appropriate, since often the class of
  the liveness properties is mathematically characterized exactly as
  that of those properties that cannot be checked within any finite
  length run. Refer, e.g., to Chapter~3 of \cite{BaKG08}
  for details.

\item ``Response'':  $\Box(\psi\limp\Diamond\varphi)$ means: always, before the end of the trace,
if $\psi$ holds then later $\varphi$ holds.

\end{itemize}



\paragraph{Transforming \LTLf formulas into \NFA's and \DFA's.}
We can associate with each \LTLf formula $\varphi$ an (exponential)
\NFA $A_\varphi$ that accepts exactly the traces that make $\varphi$
true.  
Here, we provide a simple direct algorithm for computing the \NFA
corresponding to an \LTLf formula.
The correctness of the algorithm is based on the fact that \myi we can
associate with each \LTLf formula $\varphi$ a polynomial
\emph{alternating automaton on words} (\AFW)
$\A_\varphi$ that accept exactly the traces that make $\varphi$ true
\cite{DegVa13}, and \myii every \AFW can be transformed into an
\NFA, see, e.g., \cite{DegVa13}. %\cite{BL80,CKS81,Lei81}.
 %%
However, to formulate the algorithm we do not need these notions, but
we can work directly on the \LTLf formula.
%%
We assume our formula to be in \emph{negation normal form}, by
exploiting abbreviations and pushing negation inside as much as
possible, leaving it only in front of propositions
(any \LTLf formula can be transformed into negation normal form in
linear time). 
We also assume $\Prop$ to include a special proposition
$\Last$ which denotes the last element of the trace.  Note that
$\Last$ can be defined as $\Last\equiv \Wnext\false$.
%%
%%
Then we define an auxiliary function $\delta$ that takes an \LTLf
formula $\psi$  (in negation normal form) and a propositional
interpretation $\Pi$ for $\Prop$ (including $\Last$), returning a positive
boolean formula whose atoms are (quoted) $\psi$ subformulas.
%%
\begin{comment}
The key idea in building the \AFW $\A_\varphi$ is to use
``subformulas'' as states of the automaton and generate suitable
transitions that mimic the meaning of such formulas.
%%
Actually we need a generalization of the notion of subformulas, which
is known as the Fisher-Ladner closure, first introduced in the context
of \PDL \cite{FiLa79}.  The Fisher-Ladner closure $\CL_{\varphi}$ of
an \LTLf formula $\varphi$ is a set of \LTLf formulas inductively
defined as follows:
%%
\[\begin{array}{l}
  \varphi \in \CL_{\varphi}\\
  \lnot \psi \in \CL_{\varphi} \mbox{ if } \psi\in \CL_{\varphi} \mbox{ and } \psi \mbox{ not of the form }\lnot \psi'\\
  \varphi_1 \land \varphi_2 \in \CL_{\varphi} \mbox{ implies } \varphi_1, \varphi_2 \in \CL_{\varphi}\\
  \Next\varphi'\in\CL_{\varphi} \mbox{ implies } \varphi' \in \CL_{\varphi}\\
  \Wnext\varphi'\in\CL_{\varphi} \mbox{ implies } \varphi' \in \CL_{\varphi}\\
  \Diamond\varphi' \in \CL_{\varphi} \mbox{ implies } \varphi'\in \CL_{\varphi} \mbox{ and } \Next\Diamond\varphi' \in \CL_{\varphi}\\
  \Box\varphi' \in \CL_{\varphi} \mbox{ implies } \varphi' \in \CL_{\varphi} \mbox{ and } \Wnext\Box\varphi' \in \CL_{\varphi}\\
  \varphi_1 \Until \varphi_2 \in \CL_{\varphi} \mbox{ implies } \varphi_1, \varphi_2 \in \CL_{\varphi} \mbox{ and } \Next(\varphi_1 \Until \varphi_2) \in \CL_{\varphi}\\
  \varphi_1 \Release \varphi_2 \in \CL_{\varphi} \mbox{ implies } \varphi_1, \varphi_2 \in \CL_{\varphi} \mbox{ and } \Wnext(\varphi_1 \Release \varphi_2) \in \CL_{\varphi}\\
\end{array}
\]
Observe that the cardinality of $\CL_\varphi$ is linear in the size of
$\varphi$.
%%

In order to proceed with the construction of the \AFW $\A_\varphi$, we
put \LTLf formulas $\varphi$ in negation normal form $\nnf(\varphi)$
by exploiting abbreviations and pushing negation inside as much as
possible, leaving negations only in front of propositional symbols.
Note that computing $\nnf(\varphi)$ can be done in linear time. So, in
the following, we restrict our attention to \LTLf formulas in negation
normal form, i.e., \LTLf formulas formed according to the following
syntax:

\[\begin{array}{lcl}
  \varphi &::=& a \mid \lnot a  \mid (\varphi_1 \land \varphi_2) \mid 
  (\varphi_1 \lor \varphi_2)  \mid \Next\varphi \mid \Wnext\varphi \mid {}\\
  & &\Diamond\varphi\mid \Box\varphi \mid \varphi_1\Until\varphi_2 \mid \varphi_1\Release\varphi_2
\end{array}
\]

We assume that all the formulas in $\CL_{\varphi}$ are in negation
normal form as well.  
%%
Then, we define the \AFW $\A_\varphi$ associated with an \LTLf formula
$\varphi$ as $\A_\varphi=(2^\Prop,\S,\varphi,\delta,\F)$ where
\begin{itemize}
\item $2^\Prop$ is the alphabet,
\item $\S=\CL_{\varphi}$ %\cup\{\ttrue,\ffalse\}$
  is the the state set,
\item $\varphi$ is the initial state
\item $\F=\emptyset$
\item $\delta$ is the transition function defined as follows ($\Pi$
  stands for the current letter on the word):
\end{itemize}
\end{comment}
%%

\allowdisplaybreaks
\[
\footnotesize
  \begin{array}{@{}l@{\ }c@{\ }l@{}}
    \delta(\atomize{a},\Pi) &=& \true \mbox{ if } a\in \Pi\\
     \delta(\atomize{a},\Pi) &=& \false \mbox{ if } a\not\in \Pi\\
     \delta(\atomize{\lnot a},\Pi) &=& \false \mbox{ if } a\in \Pi\\
     \delta(\atomize{\lnot a},\Pi) &=& \true \mbox{ if } a\not\in \Pi\\
     \delta(\atomize{\varphi_1\land\varphi_2},\Pi) &=& 
     \delta(\atomize{\varphi_1},\Pi) \land \delta(\atomize{\varphi_2},\Pi)\\
\delta(\atomize{\varphi_1\lor\varphi_2},\Pi) &=& 
    \delta(\atomize{\varphi_1},\Pi) \lor \delta(\atomize{\varphi_2},\Pi)\\
    \delta(\atomize{\Next\varphi},\Pi) &=&
      \begin{cases}
        \atomize{\varphi} & \mbox{ if $\Last\not\in\Pi$}\\
        \false & \mbox{ if  $\Last\in\Pi$}
      \end{cases}\\
   \delta(\atomize{\Diamond\varphi},\Pi) &=& \delta(\atomize{\varphi},\Pi) \lor \delta(\atomize{\Next\Diamond\varphi},\Pi)\\
     \delta(\atomize{\varphi_1\Until \varphi_2},\Pi) &=& \delta(\atomize{\varphi_2},\Pi) \lor {}\\
&& (\delta(\atomize{\varphi_1},\Pi) \land \delta(\atomize{\Next(\varphi_1\Until\varphi_2)},\Pi))\\
    \delta(\atomize{\Wnext\varphi},\Pi) &=&
      \begin{cases}
        \atomize{\varphi} & \mbox{ if $\Last\not\in\Pi$}\\
        \true & \mbox{ if  $\Last\in\Pi$}
      \end{cases}\\
%   \end{array}
%\]
%\[  
%  \begin{array}{@{}l@{\ }c@{\ }l@{}}
     \delta(\atomize{\Box\varphi},\Pi) &=& \delta(\atomize{\varphi},\Pi) \land \delta(\atomize{\Wnext\Box\varphi},\Pi)\\
     \delta(\atomize{\varphi_1\Release\varphi_2},\Pi) &=& \delta(\atomize{\varphi_2},\Pi) \land (\delta(\atomize{\varphi_1},\Pi) \lor {}\\
&&\delta(\atomize{\Wnext(\varphi_1\Release\varphi_2)},\Pi))
   \end{array}
   \]

\begin{comment}
\begin{itemize}
\item $2^\Prop$ is the alphabet,
\item $\S=\CL_{\varphi}\cup\{\final\}$
  is the the state set,
\item $\varphi$ is the initial state
\item $\delta$ is the transition function defined as follows ($\Pi$
  stands for the current letter on the word):

\[
  \begin{array}{lcl}
    \delta(a,\Pi) &=& 
    \left\{
      \begin{array}{l}
        \true\quad \mbox{ if $a\in \Pi$ and $\Last\not\in\Pi$}\\
        \final \quad \mbox{ if  $a\in \Pi$ and $\Last\in\Pi$}\\
       \false \mbox{ if } a\not\in \Pi
      \end{array}
    \right.\\


      \delta(\lnot a,\Pi) &=&


\left\{
      \begin{array}{l}
        \true\quad \mbox{ if $a\not \in \Pi$ and $\Last\not\in\Pi$}\\
        \final \quad \mbox{ if $a\not\in \Pi$ and $\Last\in\Pi$}\\
        \false \mbox{ if } a \in \Pi
      \end{array}
    \right.\\
   \delta(\varphi_1\land\varphi_2,\Pi) &=& 
    \delta(\varphi_1,\Pi) \land \delta(\varphi_2,\Pi)\\
    \delta(\varphi_1\lor\varphi_2,\Pi) &=& 
    \delta(\varphi_1,\Pi) \lor \delta(\varphi_2,\Pi)\\
    \delta(\Next\varphi,\Pi) &=& \left\{
      \begin{array}{l}
        \varphi\quad \mbox{ if $\Last\not\in\Pi$}\\
        \false \quad \mbox{ if  $\Last\in\Pi$}
      \end{array}
    \right.\\
    \delta(\Diamond\varphi,\Pi) &=& \delta(\varphi,\Pi) \lor \delta(\Next\Diamond\varphi,\Pi)\\
    \delta(\varphi_1\Until \varphi_2,\Pi) &=& \delta(\varphi_2,\Pi) \lor (\delta(\varphi_1,\Pi) \land \delta(\Next(\varphi_1\Until\varphi_2),\Pi))\\

    \delta(\Wnext\varphi,\Pi) &=& \left\{
      \begin{array}{l}
        \varphi\quad \mbox{ if $\Last\not\in\Pi$}\\
        \true \quad \mbox{ if  $\Last\in\Pi$}
      \end{array}
    \right.\\
    \delta(\Box\varphi,\Pi) &=& \delta(\varphi,\Pi) \land \delta(\Wnext\Box\varphi,\Pi)\\
    \delta(\varphi_1\Release\varphi_2,\Pi) &=& \delta(\varphi_2,\Pi) \land (\delta(\varphi_1,\Pi) \lor \delta(\Wnext(\varphi_1\Release\varphi_2),\Pi))
  \end{array}
  \]
\item $\F=\final$.

\end{itemize}
\end{comment}


 
\begin{comment}
Alternating automata can be translated into equivalent
nondeterministic ones. Actually in our case we do not even need to
build explicitly the \AFW, instead we use directly the rules for the
construction of the \AFW transition relation $\delta$ to build the
\NFA $\A_\varphi$ of an \LTLf formula $\varphi$ in a forward fashion as
shown in Figure~\ref{fig:algo}.
\end{comment}

\noindent Using function $\delta$ we can build the \NFA
$\A_\varphi$ of an \LTLf formula $\varphi$ in a forward fashion.
States of $\A_\varphi$ are sets of atoms (recall that each atom is
quoted $\varphi$ subformulas) to be interpreted as a conjunction; the
empty conjunction $\emptyset$ stands for $\true$:
% as
% shown in Figure~\ref{fig:algo}.


\algrenewcommand\algorithmicindent{1em}

\smallskip
\fbox{
\begin{minipage}{7.5cm}
  \begin{algorithmic}[1]
    \small 
\State\textbf{algorithm} \algoname() \\\textbf{input} \LTLf formula
    $\varphi$ \\\textbf{output} \NFA $\A_\varphi =
    (2^\Prop,\S,\{s_0\},\varrho,\{s_f\})$ 
 \State $s_0  \gets \{\atomize{\varphi}\}$
    \Comment{single initial state} 
  \State $s_f \gets \emptyset$ \Comment{single final state}  
  \State $\S \gets \{s_0,s_f\}$, $\varrho \gets \emptyset$ 
 \While{($\S$ or $\varrho$ change)} %\{
\If{($q\in \S$ and $q'\models
      \bigwedge_{(\atomize{\psi}\in q)} \delta(\atomize{\psi},\Pi)$)}

    \State $\S \gets \S \cup \{q'\}$ \Comment{update set of states}
    \State $\varrho \gets \varrho \cup
   \{ (q,\Pi,q')\}$ \Comment{update transition relation}
    \EndIf 
    \EndWhile
 %\State \} 
 %   \EndFunction
%\noindent
 \end{algorithmic} 
\end{minipage}
}

\smallskip
\noindent where $q'$ is a set of quoted subformulas of $\varphi$ that denotes a
minimal interpretation such that $q'\models \bigwedge_{(\atomize{\psi}\in q)} \delta(\atomize{\psi},\Pi)$. (Note: we do not need to get all $q$ such that
$q'\models \bigwedge_{(\atomize{\psi}\in q)} \delta(\atomize{\psi},\Pi)$,
but only the minimal ones.)  Notice that trivially we have
$(\emptyset,a,\emptyset)\in\varrho$ for every $a\in\Sigma$.
%%
\begin{comment}
\begin{figure}[!t]
  \begin{algorithmic}[1]
    \small \Function{build-\NFA}{} \\\textbf{input} \LTLf formula
    $\varphi$ \\\textbf{output} \NFA $\A_\varphi =
    (2^\Prop,S,s^0,\rho,\F)$ 
    \State $s^0 \gets \varphi$
    %\Comment{Single initial state} 
    \State $\F\gets \{\true,\final\} \mbox{ ($\true$ stands for $\emptyset$ -- empty set of atoms)}$
    %\Comment{Single final state} 
   \State $ S \gets
    \{s^0,s^f,\final\}$, $\rho \gets \emptyset$ 
 \While{($S$ or $\rho$ change)} %\{
\If{($T\in S$ and $T'\models
      \bigwedge_{t\in T} \delta(t,\Pi)$)}

    \State $S \gets S \cup \{T'\}$ \Comment{update set of states}
    \State $\rho \gets \rho \cup
    (T,\Pi,T')$ \Comment{update transition relation}
    \EndIf 
    \EndWhile
 %\State \} 
    \EndFunction

\medskip
\noindent
where $T'$ is a
      conjunction of formulas (considered as atoms) in the
      Fisher-Ladner closure $\CL(\varphi)$. Note: we do not need to
      get all $T'$ such that $T'\models \bigwedge_{t\in T}
      \delta(t,\Pi)$, but only the minimal ones.  Notice that trivially we have
    $(\true,a,\true)\in\rho$ for every $a\in\Sigma$.
  \end{algorithmic}
  \vspace{-.3cm}
  \caption{\NFA construction }\label{alg:ts}
\end{figure}
\end{comment}
%%

The algorithm  \algoname\ terminates in at most
exponential number of steps, and generates a set of states $\S$ whose size
is at most exponential in the size of the formula $\varphi$.
%%

Notice that above we have assumed to have a special proposition $\Last\in\Prop$.
If we want to remove such an assumption, we can easily transform the obtained automaton $\A_\varphi =
     (2^\Prop,\S,\{\atomize{\varphi}\},\varrho,\{\emptyset\})$ into the new automaton 
\[\A'_\varphi =
    (2^{\Prop-\{\Last\}},\S\cup\{\textit{ended}\},\{\atomize{\varphi}\},\varrho',\{\emptyset, \textit{ended}\})\] where:
$(q, \Pi', q') \in \varrho'$ iff $(q, \Pi', q')\in\varrho$, or $(q, \Pi'\cup\{\Last\}, \true) \in \varrho$ and $q'=\textit{ended}$.


The \NFA $\A_\varphi$
  constructed as above correctly capture the formula $\varphi$ in the sense that, for  every finite trace $\pi$:
 \[\pi\models\varphi \mbox{ iff } \pi\in L(\A_\varphi).\]
 
Finally we can transform the \NFA $\A_\varphi$ into a \DFA following standard construction  in exponential time, and the possibly minimize, putting it in minimal form (which is unique) it polynomial time \cite{RaSc59}. Hence overall we can transform any \LTLf formula into a \DFA of double exponential size. Notice however that this is a worst case complexity, and in most cases the size of the \DFA is actually quite manageble \cite{TaVa05}.  


\clearpage

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> 3-mdp-basic.tex <==
\clearpage
\section{Basic Setting: Complete Traces}\label{sec:mdb-basic}

\paragraph{Problem.}
We are given a (planning) domain in terms of a probabilistic transition system
%%
\[\T = (A, T, t_0, \tau)\]
%%
where: 
\begin{itemize}
\item $A$ is the set of actions;
\item $T=2^{\Prop}$ is the set of states; 
\item $t_0\in T$ is the initial state; 
\item $\tau: T\times A \times T \rightarrow [0,1]$ is the probabilistic transition function.
\end{itemize}
We assume that $A$ includes a special deterministic action $\Stop$ with no effects, i.e., $\tau(t,\Stop,t) = 1$ and $\tau(t,\Stop,t') = 0$ for all $t'\neq t$.

\smallskip
Then we  are given $\varphi_1,\ldots,\varphi_m$ \LTLf/\LDLf formulas standing for (soft) goals, each with a reward  $\rew(\varphi_i) = r_i$.

Our problem is to find a \emph{policy that maximizes expected
  discounted rewards on the compete traces}. \todo{How do we state the
  problem formally?}
%%
A \emph{complete trace} is a sequence of the form $t_0 a_1, t_1 a_2 \cdots t_{n-1} a_n, t_n$ such that
\begin{itemize}
\item $a_k = \rho(t_0,\ldots t_{k-1})$;
\item $t_{k-1} a_k t_k$ implies $\tau(t_{k-1}, a_k, t_k)\neq 0$;
\item $a_n = \Stop$ and $a_i \neq \Stop$ for $i<n$.
\end{itemize}
The trace $t_0 a_1, t_1 a_2 \cdots t_{n-1} a_n, t_n$ gets $rew(\varphi_i)$ iff $t_0 t_1 \cdots t_{n-1} \models\varphi_i$. 


\paragraph{Solution.}
For each of goal formula $\varphi_i$ we consider the corresponding (minimal) \DFA
%%
\[\A_{\varphi_i} = (2^{\Prop\cup\{\Last\}}, Q_i, q_{io}, \delta_i,F_i)\] 
%%
where:
\begin{itemize}
\item $2^{\Prop\cup\{\Last\}}$ is the input alphabet of the automaton, we included $\Last$ to denote the last element of a trace for convenience;
\item $Q_i$ is the finite set of states ;
\item $q_{io} \in Q_i$ is the initial state;
\item $\delta_i:Q\times 2^\Prop\rightarrow Q$ is the deterministic transition function
(which is total); 
\item $F_i\subseteq Q_i$ are the accepting
states.
\end{itemize}

\smallskip
Now for solving the problem we build the \MDP 
\[\M = (S, A, \Tr, R)\] 
where:
\begin{itemize}
\item $S=Q_1\times\cdots\times Q_m\times T$ is the set of states;
\item $A$ is the set of actions which are the one of the domain;
\item $\Tr: Q_1\times\cdots\times Q_m\times T\times A \times Q_1\times\cdots\times Q_m \times T\rightarrow [0,1]$ is the \MDP probabilistic transition function, defined as:
\[
\begin{array}{l}
\Tr(q_1,\ldots,q_m, t, a, q'_1,\ldots,q'_m, t') = {}\\
\quad\left\{
\begin{array}{ll}
\tau(t,a,t') &\mbox{if } \delta(q_i,t) = q'_i \mbox{ and } a\neq\Stop\\
\tau(t,a,t') &\mbox{if } \delta(q_i,t\cup\{\Last\}) = q'_i \mbox{ and } a=\Stop\\
0 & \mbox{otherwise}; 
\end{array}\right.
\end{array}
\] 
\item $R: Q_1\times\cdots\times Q_m\times T\times A\rightarrow 
\mathbb{R}$ is the \MDP reward function, defined as:
\[
\begin{array}{l}
R(q_1,\ldots,q_m, t, a) = {}\\
\quad\left\{
\begin{array}{ll}
\sum_i \{\rew(\Phi_i) \mid \delta(q_i,t\cup\{\Last\}) \in F_i\} & \mbox{if } a=\Stop\\
0 & \mbox{otherwise}.
\end{array}\right.
\end{array}
\] 
\end{itemize}
\todo{Can $\A_1\times\cdots\times \A_m$ be minimized? If we did not need to keep track of the final states separately YES, but we do so NO! The automata are completely orthogonal!}
\todo{Is it possible to compute $\A_1\times\cdots\times \A_m$ from $\varphi_1,\cdots,\varphi_m$ on-the-fly? Possibly! But we need to avoid minimization of the single \DFA's.}

We can obtain an optimal policy $\rho_\M: S\rightarrow A$ solving the \MDP $\M$ by considering a discount factor $\gamma$ \todo{Where does $\gamma$ come from?}. From  $\rho_\M$ we get the policy solving our original problem by  observing that by executing  any (possibly partial) trace $t_0 a_1, t_1 a_2 \cdots t_{k-1} a_k, t_k$ we get a single state $exec(t_0 a_1, t_1 a_2 \cdots t_{k-1} a_k, t_k) = s$ of the \MDP. 

\clearpage
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> 4-mdp-monitoring.tex <==
\section{Adding Monitoring}
Diverse solution methods can be used with our NMRDPs. Methods based on
dynamic programming, requiring state enumeration will benefit from our
ability to minimize the resulting MDP.  Methods based on forward
search will benefit from the ability to construct the extended MDP
incrementally using progression. Of particular interest are methods
that are able to exploit the existence of multiple independent
components. Indeed, note that the component of the state that
corresponds to $\A_{\varphi_i}$ is independent of other components --
it does not affect them nor does it next state depend on them. This
structure was exploited in the past, e.g., by Meuleau et al.~\cite{}.

However, one problem with non-Markovian rewards is that the reward is
only obtained when the entire sequence satisfies the property. This is
especially true if we wish to give rewards for complete traces only.
In that case, the reward come as a "surprise" when the last action
$\Stop$ is chosen.  We can help solution algorithms if we can start
rewarding such behaviors even before the formula is satisfied, helping
to guide both search and learning algorithms towards better behaviors.

To do so we relay on notions coming from monitoring.  Monitoring
amounts to observing the evolving system execution and reporting the
violation or satisfaction of properties of interest at the earliest
possible time. As the system progresses, its execution trace
increases, and at each step the monitor checks whether the trace seen
so far conforms to the property \cite{Bauer2010:LTL}.  

Specifically, following \cite{DDGMM-BPM14,MMW11}, we adopt a the
finite-trace variant of the well-known RV semantics in
\cite{Bauer2010:LTL}.
%%
For a \LTLf/\LDLf formula $\varphi_i$, each time the system evolves,
the monitor returns one among the following truth values:
\begin{itemize}
\item $ [\varphi_i]_{RV}=\temptrue$, meaning that the current execution trace \emph{temporarily satisfies} $\varphi_i$, i.e.,
  it is currently compliant with $\varphi_i$, but there is a
  possible system future prosecution which may lead to falsify $\varphi_i$;

\item $[\varphi_i]_{RV}=\tempfalse$, meaning that the current trace  \emph{temporarily falsify} $\varphi_i$, i.e.,
  $\varphi_i$ is not current compliant with $\varphi_i$, but there is a
  possible system future prosecution which may lead to satisfy $\varphi_i$;

\item $ [\varphi_i]_{RV}=\willtemptrue$, meaning that the current execution trace will eventually \emph{temporarily satisfies} $\varphi_i$, i.e.,
  no matter how the process develops, it will reach a point where $\varphi_i$ is satisfied, but there is a
  possible system future prosecution which may then lead to falsifying $\varphi_i$;

\item $[\varphi_i]_{RV}=\true$, meaning that the current trace  \emph{satisfies} $\varphi_i$ and it will always do,
  no matter how it proceeds;

\item $[\varphi_i]_{RV}=\false$, meaning that the current trace  \emph{falsifies} $\varphi_i$ and it will always do,
  no matter how it proceeds.
  
\item $[\varphi_i]_{RV}=\willtrue$, meaning that, if allowed to continue for a sufficient number of steps, no matter
how it proceeds, the trace will eventually \emph{satisfy} $\varphi_i$ and continue to do so form that point on.

\item $[\varphi_i]_{RV}=\willfalse$, meaning that, if allowed to continue for a sufficient number of steps, no matter
how it proceeds, the trace will eventually  \emph{falsify} $\varphi_i$ and continue to do so form that point on.

\end{itemize}
The first two conditions are unstable because they may change into any
other value as the system progresses.  The third condition allows us to
reward a state that will necessarily lead to a reward.
The last four conditions are stable since, once outputted, they will not change
anymore. 
%This can happen either when the system execution has
%terminated ($\Last$ is met) or when the formula that is being
%monitored $\varphi_i$ can be fully evaluated by observing the current
%partial trace only.
%%
Notice that in the latter case, it is irrelevant whether the systems
continues its execution or not, since the truth value of $\varphi_i$
is already determined.

In practice, to do monitoring of a formula $\varphi_i$ it is enough to build the automata $\A_{\varphi_i} $ for formula $\varphi_i$  then \emph{color} its states properly \cite{DDGMM-BPM14,MMW11}. 
%%
The procedure is follows. Let $\A_{\varphi_i} = (2^{\Prop\cup\{\Last\}}, Q_i, q_{io}, \delta_i,F_i)$. We denote by $Reach(q)$ the states in $Q_i$ that are reachable from $q$. Note that checking reachability is linear (in fact \NLOGSPACE) in the size of the automaton $\A_{\varphi_i}$. Then we mark the states $q$ of $\A_{\varphi_i}$, by matching the seven monitoring conditions above, as follows:
\begin{itemize}
\item if $q \in F_i$ and $Reach(q) \not \subseteq F_i$ and $Reach(q) \cap F_i\not = \emptyset$, then we mark $q$ as $\temptrue$;
\item if $q \not \in F_i$ and $Reach(q) \not \subseteq (Q_i \setminus F_i)$ and $Reach(q) \cap F_i \not = \emptyset$, then we mark $q$ as $\tempfalse$;
\item if $q \not\in F_i$ and ...
\item if  $q \in F_i$ and $Reach(q) \subseteq F_i$ then we mark $q$ as $\true$;
\item if $q \not \in F_i$ and $Reach(q) \subseteq (Q_i \setminus F_i)$ then we mark $q$ as $\false$.
\item if 
\item if 
\end{itemize}
In some of the above cases, it is possible to attempt to change the reward definition so that behaviors are rewarded earlier, without affecting the value of a complete trace (and hence, without changing the optimal policy). In particular, cases $\willtemptrue,\willtrue$, we
can reward this behavior once these conditions are satisfied, rather than later when the formula is satisfied.%
\footnote{This may require maintaining additional information in the state to detect the {\em first} time the condition is satisfied.
In the case of $\willtrue$ we may also need to mark the first state in which it becomes $\true$.}

In the case where rewards are defined for complete traces only, one can also handle $\false$ and $\willfalse$. 
Suppose that if $\varphi$ becomes true then reward $r$ is obtained.
We can, instead, give a reward of $-r$ when $\willfalse$ or $\false$ become true, and give 0 reward the first
time the condition becomes true. We must also give $-r$ at the end of the trace if $\varphi$ is not true
and $\willfalse$ was never true in the trace.  Although the reward of the complete trace is now changed, the reward of
every trace is changed by a constant, and hence the optimal policy remains optimal.
There is a caveat, however. If discounting is used, then earlier rewards are more valuable (or harmful, if negative) than later
rewards, and this can affect the identity of the optimal policy.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> macro/environments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Time-stamp: "2012-10-10 18:54:10 savo"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%    TO-DO NOTES Domenico Fabio Savo
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\definecolor{notecolor}{rgb}{0.4,0,0}
%%\newcommand{\todo}[1]{\par\noindent\framebox{\parbox{\columnwidth}{\textcolor{notecolor}{\textbf{#1}}}}\par}
%
%  \newcommand{\todo}[1]{
%    \addcontentsline{tdo}{todo}{\protect{#1}}
%    %marginpar{#1}
%    \par\noindent\framebox{\parbox{\columnwidth}{\textcolor{notecolor}{\textbf{#1}}}}\par
%}
%
%%% per visualizzare la to-do-list
%
%\makeatletter \newcommand \listoftodos{\section*{Todo list} \@starttoc{tdo}}
%  \newcommand\l@todo[2]
%    {\par\noindent \textit{#2}, \parbox{10cm}{#1}\par} \makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%ANTONELLA: ambiente con riquadro
\newsavebox{\fmbox}
   \newenvironment{fmpage}[1]
     {\begin{lrbox}{\fmbox}\begin{minipage}{#1}}
     {\end{minipage}\end{lrbox}\fbox{\usebox{\fmbox}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%% USEFUL

\newcommand{\titleconference}[3]{\title{\hspace*{\fill}%
 \begin{minipage}[t]{\textwidth} \centering #1 \end{minipage}%
 \hspace*{\fill}\makebox[0cm][r]{\raisebox{#2}[0cm][0cm]{\small\textmd{#3}}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%% ENVIRONMENTS and THEOREMS

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}

\newtheorem{definitionAux}{Definition}
\newenvironment{definition}{\begin{definitionAux}\rm}{\end{definitionAux}}

\newtheorem{claimAux}{Claim}
\newenvironment{claim}{\begin{claimAux}\rm}{\end{claimAux}}

\newtheorem{exampleAux}{Example}
\newenvironment{example}{\begin{exampleAux}\rm}{\end{exampleAux}}
\newenvironment{exampleCont}[1]{\trivlist
\item[\hskip \labelsep{\textbf{Example~#1 (contd.)}}]}{\endtrivlist}

\newtheorem{examplesAux}{Examples}
\newenvironment{examples}{\begin{examplesAux}\rm}{\end{examplesAux}}

\newtheorem{constructionAux}{Construction}
\newenvironment{construction}{\begin{constructionAux}\rm}
                             {\end{constructionAux}}

\newenvironment{proof}{\noindent \textsl{Proof.\ }}{\qedfull}
\newenvironment{proofsk}{\noindent \textsl{Proof (sketch).\ }}{\qedfull}

%\newcommand{\Proof}{\textsl{Proof.\ }}
%\newcommand{\Proofsk}{\textsl{Proof (sketch).\ }}

\long\def\eatpar#1{%
\ifx#1\par                      % se il token e' \par
\let\nextmove=\eatpar           % rimetti \eatpar in coda
\else
\let\nextmove=#1%               altrimenti, rimetti il token in coda
\fi
\nextmove%                      il token o \eatpar viene rimesso in coda
}

\def\qed{\hfill{\qedboxempty}      % qed with empty box
  \ifdim\lastskip<\medskipamount \removelastskip\penalty55\medskip\fi}

\def\qedboxempty{\vbox{\hrule\hbox{\vrule\kern3pt
                 \vbox{\kern3pt\kern3pt}\kern3pt\vrule}\hrule}}

\def\qedfull{\hfill{\qedboxfull}   % qed with full box
  \ifdim\lastskip<\medskipamount \removelastskip\penalty55\medskip\fi}

\def\qedboxfull{\vrule height 4pt width 4pt depth 0pt}

\newcommand{\markfull}{\qedfull}
\newcommand{\markempty}{\qed}

%\newcommand{\If}{\lq\lq$\Leftarrow$\rq\rq\ \ }           % 1st direction of iff
%\newcommand{\OnlyIf}{\lq\lq$\Rightarrow$\rq\rq\ \ }      % 2nd direction of iff

%%%%%%%%%%%%%%%%%%%%%%%%%%% BOXES

\newcommand{\fpbox}[3]{\framebox[#1]{\parbox{#2}{#3}}}
\newcommand{\boxtext}[1]{\fpbox{\textwidth}{0.9\textwidth}{#1}}
\newcommand{\boxcolumn}[1]{\fpbox{\columnwidth}{0.9\columnwidth}{#1}}
\newcommand{\boxformula}[1]{%
  \vspace{\abovedisplayskip}
  \boxtext{\vspace{-\abovedisplayskip} #1 \vspace{-\abovedisplayskip}}
  \vspace{\abovedisplayskip}}

%%%%%%%%%%%%%%%%%%%%%%%%%%% OTHERS

\newcommand{{\incolumn}}[1]{\begin{tabular}[c]{c} #1 \end{tabular}}
\newcommand{{\incolumnmath}}[1]{\begin{array}[c]{c} #1 \end{array}}
%% note: "x \atop y" may be more convenient

%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% save-place: t
%%% End:


==> macro/macro-todo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%    TO-DO NOTES Domenico Fabio Savo
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{color}
\definecolor{notecolor}{rgb}{0.4,0,0}
\newcommand{\todo}[1]{
    \addcontentsline{tdo}{todo}{\protect{#1}}
    %marginpar{#1}
\ \newline \par\noindent\framebox{\parbox{\columnwidth}{  \textcolor{notecolor}{\textbf{#1}}}}\par}

%%% per visualizzare la to-do-list

\makeatletter \newcommand \listoftodots{\section*{To-do list} \@starttoc{tdo}}
  \newcommand\l@todo[2]
    {\par\noindent \textit{#2}, \parbox{10cm}{#1}\par} \makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{refcolor}{rgb}{0.6,0,0}
\definecolor{seccolor}{rgb}{0.13,0.54,0.13}
\definecolor{urlc}{rgb}{0,0,1} 

==> macro/macros-2012.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Time-stamp: "11/10/2012 19:16:00 savo"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\myi}{(\emph{i})\xspace}
\newcommand{\myii}{(\emph{ii})\xspace}
\newcommand{\myiii}{(\emph{iii})\xspace}
\newcommand{\myiv}{(\emph{iv})\xspace}
\newcommand{\myv}{(\emph{v})\xspace}
\newcommand{\myvi}{(\emph{vi})\xspace}
\newcommand{\myvii}{(\emph{vii})\xspace}
\newcommand{\myviii}{(\emph{viii})\xspace}

\newcommand{\A}{\mathcal{A}} \newcommand{\B}{\mathcal{B}}
\newcommand{\C}{\mathcal{C}} \newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathcal{E}} \newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}} \renewcommand{\H}{\mathcal{H}}
\newcommand{\I}{\mathcal{I}} \newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}} \renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}} \newcommand{\N}{\mathcal{N}}
\renewcommand{\O}{\mathcal{O}} \renewcommand{\P}{\mathcal{P}}
\newcommand{\Q}{\mathcal{Q}} \newcommand{\R}{\mathcal{R}}
\renewcommand{\S}{\mathcal{S}} \newcommand{\T}{\mathcal{T}}
\newcommand{\U}{\mathcal{U}} \newcommand{\V}{\mathcal{V}}
\newcommand{\W}{\mathcal{W}} \newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}} \newcommand{\Z}{\mathcal{Z}}
\newcommand{\DB}{\D\B}

%%%%%%%%%%%%%%%%%%%%%%%%%% Abbreviations

\newcommand{\setone}[2][1]{\set{#1\cld #2}}
\newcommand{\eset}{\emptyset}
%%\newcommand{\col}{\colon}
\newcommand{\ol}[1]{\overline{#1}}                % overline
\newcommand{\ul}[1]{\underline{#1}}               % underline
\newcommand{\uls}[1]{\underline{\raisebox{0pt}[0pt][0.45ex]{}#1}}
\newcommand{\wrt}{w.r.t.\xspace}
\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Lra}{\Leftrightarrow}
\newcommand{\lora}{\longrightarrow}
\newcommand{\Lora}{\Longrightarrow}
\newcommand{\lola}{\longleftarrow}
\newcommand{\Lola}{\Longleftarrow}
\newcommand{\lolra}{\longleftrightarrow}
\newcommand{\Lolra}{\Longleftrightarrow}
\newcommand{\ua}{\uparrow}
\newcommand{\Ua}{\Uparrow}
\newcommand{\da}{\downarrow}
\newcommand{\Da}{\Downarrow}
\newcommand{\uda}{\updownarrow}
\newcommand{\Uda}{\Updownarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%% Relations

\newcommand{\incl}{\subseteq}
\newcommand{\imp}{\rightarrow}
%%\newcommand{\deq}{\doteq}
\newcommand{\dleq}{\dot{\leq}}                   % dotted less equal

%%%%%%%%%%%%%%%%%%%%%%%%%% Spaces

\newcommand{\per}{\mbox{\bf .}}                  % period

\newcommand{\cld}{,\ldots,}                      % ,...,
\newcommand{\ld}[1]{#1 \ldots #1}                 % #1 ... #1
\newcommand{\cd}[1]{#1 \cdots #1}                 % #1 ... #1
\newcommand{\lds}[1]{\, #1 \; \ldots \; #1 \,}    % _#1_..._#1_
\newcommand{\cds}[1]{\, #1 \; \cdots \; #1 \,}    % _#1_..._#1_

\newcommand{\dd}[2]{#1_1,\ldots,#1_{#2}}             % x1,...,xn (da da)
\newcommand{\ddd}[3]{#1_{#2_1},\ldots,#1_{#2_{#3}}}  % xi1,...,xin (da da down)
\newcommand{\dddd}[3]{#1_{11}\cld #1_{1#3_{1}}\cld #1_{#21}\cld #1_{#2#3_{#2}}}
%%                                x_11,...,x_1n,...,x_m1,...,x_mn_m

\newcommand{\ldop}[3]{#1_1 \ld{#3} #1_{#2}}   % x1 #3...#3 xn
\newcommand{\cdop}[3]{#1_1 \cd{#3} #1_{#2}}   % x1 #3...#3 xn
\newcommand{\ldsop}[3]{#1_1 \lds{#3} #1_{#2}} % x1 _#3_..._#3_ xn
\newcommand{\cdsop}[3]{#1_1 \cds{#3} #1_{#2}} % x1 _#3_..._#3_ xn

%%%%%%%%%%%%%%%%%%%%%%%%%% Delimiters

\newcommand{\quotes}[1]{{\lq\lq #1\rq\rq}}
\newcommand{\set}[1]{\{#1\}}                      % set
\newcommand{\Set}[1]{\left\{#1\right\}}
%%\newcommand{\bigset}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\bigmid}{\Big|}
\newcommand{\card}[1]{|{#1}|}                     % cardinality of a set
\newcommand{\Card}[1]{\left| #1\right|}
\newcommand{\cards}[1]{\sharp #1}
\newcommand{\sub}[1]{[#1]}
\newcommand{\tup}[1]{\langle #1\rangle}            % tuple
\newcommand{\Tup}[1]{\left\langle #1\right\rangle}
\newcommand{\inc}[2]{#1\colon #2}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DL NAMES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ----- proper names -----
\newcommand{\dllite}{\textit{DL-Lite}\xspace}
\newcommand{\dllitecore}{\textit{DL-Lite}\ensuremath{_{\mathit{core}}}\xspace}
\newcommand{\dllitehornh}{\textit{DL-Lite}\ensuremath{_{\mathit{horn}}^\H}\xspace}
\newcommand{\dllitea}{\textit{DL-Lite}\ensuremath{_{\A}}\xspace}
\newcommand{\dllitef}{\textit{DL-Lite}\ensuremath{_{\F}}\xspace}
\newcommand{\dlliter}{\textit{DL-Lite}\ensuremath{_{\R}}\xspace}
\newcommand{\alc}{\ensuremath{\A\L\C}\xspace}
\newcommand{\alchiq}{\ensuremath{\A\L\C\H\I\Q}\xspace}
\newcommand{\alchiqr}{\ensuremath{\A\L\C\H\I\Q^{\AND}}\xspace}
\newcommand{\el}{\ensuremath{\E\L}\xspace}
\newcommand{\eli}{\ensuremath{\E\L\I}\xspace}
\newcommand{\elh}{\ensuremath{\E\L\H}\xspace}
\newcommand{\elplus}{\ensuremath{\E\L^{+}}\xspace}
\newcommand{\elplusplus}{\ensuremath{\E\L^{++}}\xspace}
\newcommand{\sroiq}{\ensuremath{\S\R\O\I\Q}\xspace}
\newcommand{\sriq}{\ensuremath{\S\R\I\Q}\xspace}
\newcommand{\hshiq}{\text{Horn-}\-\ensuremath{\mathcal{SHIQ}}\xspace}
\newcommand{\hshi}{\text{Horn-}\-\ensuremath{\mathcal{SHI}}\xspace}
\newcommand{\shiq}{\ensuremath{\mathcal{SHIQ}}\xspace}
\newcommand{\shi}{\ensuremath{\mathcal{SHI}}\xspace}
\newcommand{\halchoiq}{\text{Horn-}\ensuremath{\cal{ALCHOIQ}^{\msf{Disj}}_{\msf{Self}}}\xspace}
\newcommand{\halchiq}{\text{Horn-}\ensuremath{\cl{ALCHIQ}}\xspace}
%\newcommand{\halchiqr}{\text{Horn-}\ensuremath{\cl{ALCHIQ}^\AND}\xspace}
\newcommand{\halcif}{\text{Horn-}\ensuremath{\cl{ALCIF}}\xspace}
\newcommand{\halcf}{\text{Horn-}\ensuremath{\cl{ALCF}}\xspace}
\newcommand{\owltwo}{OWL\,2\xspace}
\newcommand{\owlql}{OWL\,2\,QL\xspace}
\newcommand{\owldl}{OWL~DL\xspace}
\newcommand{\wwwc}{W3C\xspace}

\newcommand{\dlrliteand}{\textit{DLR-Lite$_{\mathcal{A},\AND}$}\xspace}
\newcommand{\dlliteaidden}{\textit{DL-Lite}_{A,id,den}\xspace}
\newcommand{\dlliteden}{\textit{DL-Lite}_{A,id,den}\xspace}
%%% complexity classes
\newcommand{\LOGSPACE}{\textsc{LogSpace}\xspace}
\newcommand{\NLOGSPACE}{\textsc{NLogSpace}\xspace}
\newcommand{\PTIME}{\textsc{PTime}\xspace}
\newcommand{\EXPTIME}{\textsc{ExpTime}\xspace}
\newcommand{\NEXPTIME}{\textsc{NExpTime}\xspace}
\newcommand{\NP}{\textrm{NP}\xspace}
\newcommand{\NPcomp}{\textrm{NP-Complete}\xspace}
\newcommand{\NPhard}{\textrm{NP-Hard}\xspace}
\newcommand{\coNP}{\textrm{coNP}\xspace}
\newcommand{\ACz}{\textsc{AC}\ensuremath{^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DLs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ALCQIb}{\mathcal{ALCQI}b}
\newcommand{\AL}{\mathcal{AL}}
\newcommand{\ALE}{\mathcal{ALE}}
\newcommand{\ALU}{\mathcal{ALU}}
\newcommand{\FLE}{\mathcal{FLE}}
\newcommand{\EL}{\mathcal{EL}}
\newcommand{\SHIQ}{\mathcal{SHIQ}}
\newcommand{\ALCQIO}{\mathcal{ALCQIO}}
\newcommand{\SROIQD}{\mathcal{SROIQ}(D)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\AND}{\sqcap}
\newcommand{\OR}{\sqcup}
\newcommand{\NOT}{\neg}
\newcommand{\ALL}[2]{\forall #1 \per #2}
\newcommand{\SOME}[2]{\exists #1 \per #2}
\newcommand{\SOMET}[1]{\exists #1}
\newcommand{\ALLRC}{\ALL{R}{C}}
\newcommand{\SOMERC}{\SOME{R}{C}}
\newcommand{\SOMERT}{\SOMET{R}}
\newcommand{\ATLEAST}[2]{(\geq #1 \, #2)}
\newcommand{\ATMOST}[2]{(\leq #1 \, #2)}
\newcommand{\ATLEASTT}[3]{\geq #1 \, #2 \per #3}
\newcommand{\ATMOSTT}[3]{\leq #1 \, #2 \per #3}
\newcommand{\EXACTLY}[2]{(= #1 \, #2)}
\newcommand{\INV}[1]{#1^{-}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% MACROS-I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\atom}[3][]{\gamma_{#1}(#2,#3)}
\newcommand{\ISA}{\sqsubseteq}
\newcommand{\EQU}{\equiv}
\newcommand{\IMP}{\mathop{\Ra}}
\newcommand{\DIFF}{\setminus}
\newcommand{\COMP}[2]{\$#1\mathop{:}#2}
\newcommand{\QATLEAST}[3]{(\geq #1\,#2 \per\, #3)}
\newcommand{\QATMOST}[3]{(\leq #1\,#2 \per\, #3)}
\newcommand{\ID}{\mathit{id}}
\newcommand{\SOMER}[2]{\exists[\$#1]#2}
\newcommand{\ATMOSTR}[3]{(\leq #1\, [\$#2]#3)}
\newcommand{\PROJ}[3]{#1|_{#2,#3}}
\newcommand{\head}{\mathit{head}}
\newcommand{\body}{\mathit{body}}
\newcommand{\rel}[1]{\mathit{#1}}
\newcommand{\bodyl}[1][j]{\body_{#1}(\vett{a},\vett{b}_{#1},\vett{c}_{#1})}
\newcommand{\bodyr}[1][j]{\lnot\exists\vett{z}_{#1}\per
                          \body'_{#1}(\vett{a},\vett{z}_{#1},\vett{c}_{#1})}
\newcommand{\arity}[1]{\mathit{arity}(#1)}
\newcommand{\vett}[1]{\vec{\mathbf{#1}}}
\newcommand{\intsys}{\langle\G,\S,\M\rangle}
\newcommand{\true}{\textit{true}}
\newcommand{\false}{\textit{false}}
\newcommand{\vv}{\vec{v}}
\newcommand{\SemIcar}[1]{\mathit{Sem}_{\mathit{ICAR}}(#1)}
\newcommand{\ModIcar}[1]{\mathit{Mod}_{\mathit{ICAR}}(#1)}
\newcommand{\chase}{\mathit{chase}}
\newcommand{\unfold}{\mathit{unfold}}
\newcommand{\mapp}{\rho}
\newcommand{\CSP}{{\sc CSP}}
\newcommand{\UCQ}{{\sc UCQ}\xspace}
\newcommand{\UCQs}{{\sc UCQ}s\xspace}
\newcommand{\ie}{\emph{i.e.,}\xspace}
\newcommand{\eg}{\emph{e.g.,}\xspace}
%%
\newcommand{\conj}{\textit{conj}}
\newcommand{\gr}{\textit{ngr}}
\newcommand{\trasf}{\tau}
\newcommand{\ass}{\leftarrow}
%\newcommand{\ass}{:=}
\newcommand{\idrewr}{\mathsf{IDrewrite}}
\newcommand{\funct}[1]{(\mathsf{funct}\; #1)}
\newcommand{\functir}[2]{(\mathsf{funct}\; #1{:}#2)}
\newcommand{\FUNCT}[1]{(\mathsf{funct}\; #1)}
\newcommand{\KEYR}[2]{(\mathsf{key}\; #1{:}\,#2)}
\newcommand{\SOMEIRQ}[3]{\exists #1{:}#2\per #3}
\newcommand{\range}[2]{(\mathsf{range}\; #1~#2)}
\newcommand{\se}{\noindent \leftarrow}
\newcommand{\Ans}{\mathit{ans}}
\newcommand{\tab}{\mathit{tab}}
\newcommand{\aux}{\mathit{aux}}
\newcommand{\SOMEIR}[2]{\exists #1{:}#2}
\newcommand{\IR}[2]{#1{:}#2}
\newcommand{\DOMAIN}[1]{\delta(#1)}
\newcommand{\RANGE}[1]{\rho(#1)}
\newcommand{\DOMAINSEL}[2]{\delta_{#1}(#2)}
\newcommand{\topc}{\top_C}
\newcommand{\topd}{\top_D}
\newcommand{\Map}[3]{ (#1,#2,#3)}
\newcommand{\limp}{\ra}
%%%%%%%%%%%%%%%%%%%%%%%%%% Interpretation

\newcommand{\inter}[1][I]{(\dom[#1],\Int[#1]{\cdot})}   % (dom^I,.^I)
\newcommand{\dom}[1][I]{\Delta^{#1}}  % delta^I (domain of interpretation \I)
\newcommand{\domO}[1][~I]{\Delta_O^{#1}}  % delta_O^I (domain of interpretation ids)
\newcommand{\domV}[1][~I]{\Delta_V^{#1}}  % delta_V^I (domain of interpretation values)
\newcommand{\fint}[1][I]{\Int[#1]{\cdot}}
\newcommand{\Int}[2][I]{#2^{#1}}      % #2^I    (interpretation function)
%\newcommand{\IntO}[2][I]{#2^{#1,\assignO}}      % #2^I    (interpretation function)
\newcommand{\INT}[2][I]{(#2)^{#1}}    % (#2)^I  (interpretation function)
\newcommand{\IntDB}[2][\DB]{#2^{#1}}      % #2^DB    (interpretation function)
%% ANTONELLA
\newcommand{\intsysdl}{\langle\G,\C,\S,\M\rangle}
\newcommand{\IS}{\Pi}
\newcommand{\perfectref}{\textsf{PerfectRef}}
\newcommand{\assign}[1][]{\mu^{#1}}
\newcommand{\assigni}[3]{{#1}[{#2}/{#3}]}
\newcommand{\clni}[1][i]{\mathit{cln}_{#1}(\T)}
\newcommand{\NSFR}{NSFR}
\newcommand{\NI}{NI\xspace}
\newcommand{\PI}{PI\xspace}
\newcommand{\unb}{\texttt{\_}\,}
\newcommand{\crule}[1]{\textbf{cr{#1}}}
\newcommand{\dbi}[2]{\mathit{db}(#1,#2)}
\newcommand{\basic}{\textsf{KBBasicRef}}
\newcommand{\unifiedKB}{\textsf{KBUnifiedRef\xspace}}
\newcommand{\violni}{\textsf{ViolateNI}}
\newcommand{\violf}{\textsf{ViolateFunct}}
\newcommand{\assignO}{{\mu_{\bf 0}}}
\newcommand{\assignOi}[2][\assignO]{{#2}[{#1}]}
\newcommand{\Identity}{\mathit{Id}}
\newcommand{\dlliteam}{\textit{DL-Lite}_{A,M}\xspace}
\newcommand{\model}[1][M]{\inter[{#1}]}
\newcommand{\relation}[1]{\mathsf{{#1}}\xspace}
\newcommand{\rewrite}{\mathsf{RewDB}\xspace}
\newcommand{\modelsat}{\mathsf{ModelSat}\xspace}
\newcommand{\modelreach}{\mathsf{ModelReach}\xspace}
\newcommand{\clean}{\mathsf{Clean}\xspace}
\newcommand{\prdb}{\mathit{PR^{DB}}}
\newcommand{\conv}{\textsf{Conv}}
\newcommand{\GammaO}{\Gamma_O}
\newcommand{\GammaV}{\Gamma_V}
\newcommand{\modO}{I_{\bf 0}}
\newcommand{\VO}{\V_O}
\newcommand{\VV}{\V_V}
\newcommand{\bd}{\D\B}
\newcommand{\modelAss}[1][\assign]{\models_{#1}}
\newcommand{\subst}{\sigma}
\newcommand{\vx}{\vec{x}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vd}{\vec{d}}
\newcommand{\vfx}{\vec{f(x)}}
\newcommand{\vfy}{\vec{f(y)}}
\newcommand{\vfd}{\vec{f(d)}}
\newcommand{\splitted}{\textsf{Split}}
\newcommand{\sld}{\textsf{SLD-Derive}}
\newcommand{\violates}{\textsf{Violates}}
\newcommand{\size}{\textsf{size}}
\newcommand{\TEST}[1]{#1?}
\newcommand{\rma}[3]{#1(#2,#3)}
\newcommand{\length}{\mathit{length}}
\newcommand{\sig}{\mathsf{sig}}
\newcommand{\ind}{\mathsf{Ind}}

%%%%%%%%%%%%%%%%%%%%%QUERY%%%%%%%%%%%%%%%%%%%%%%
%certain answers sull'ontologia senza mappings
\newcommand{\ans}[2]{\mathit{#1^{#2}}}
%certain answers sull'ontologia con mappings
\newcommand{\ansx}[2]{\mathit{#1^{#2}}}
%query su un database
\newcommand{\ansdb}[2]{\mathit{ans(#1,#2)}}
\newcommand{\mgu}{\textit{mgu}\xspace}
\newcommand{\ontmap}{\langle \T, \M, \DB \rangle}
\newcommand{\ontmapi}{\langle \T', \M', \DB' \rangle}
\newcommand{\OM}{{\O_{m}}}
\newcommand{\db}[1][\A]{{\mathit{DB}({#1})}}
\newcommand{\cln}[1][\T]{\mathit{cln}(#1)}
\newcommand{\PerfectRef}{\textsf{PerfectRef}\xspace}
\newcommand{\pr}{\mathit{PR}}
\newcommand{\Sat}{\textsf{Sat}\xspace}
\newcommand{\Answer}{\textsf{Answer}}
\newcommand{\alltuples}{\textit{AllTup}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vxi}{\vec{x'}}
\newcommand{\directDIS}{\textsf{DirectDIS}}
\newcommand{\ComputeVSets}{\textsf{ComputeVSets}\xspace}
\newcommand{\SatisfiableIDC}{\textsf{SatisfiableIDC}\xspace}
\newcommand{\Fillers}{\textsf{Fillers}\xspace}
\newcommand{\Clash}{\emph{Clash}\xspace}
%%%updates
\newcommand{\upd}{\circ}
\newcommand{\updateM}[3][\T]{{#2}\text{\boldmath $\circ$}_{#1}{#3}}
\newcommand{\update}[3][\T]{{#2}\circ_{#1}{#3}}
\newcommand{\upmod}[3][\T]{U^{#1}({#2},{#3})}
\newcommand{\simdiff}{\ominus}
\newcommand{\resup}[3]{\mathit{ComputeUpdate}({#1},{#2},{#3})}
\newcommand{\resupshort}[0]{\mathit{ComputeUpdate}}
\newcommand{\sat}[3][\T]{\mathit{SatModel}({#1},{#2},{#3})}
\newcommand{\ALC}{\ensuremath{\mathcal{ALC}}}

%%%%%%%%PROTOTYPE%%%%%%%%%%%%%

\newcommand{\QuOnto}{\textrm{QuOnto}\xspace}
\newcommand{\styx}{\textrm{StyX}\xspace}
\newcommand{\carin}{\textrm{CARIN}\xspace}
\newcommand{\picsel}{\textrm{PICSEL}\xspace}
\newcommand{\MASTROI}{\textsc{Mastro-i}\xspace}




%%% MACROS sezione 3

\newcommand{\HB}{\textit{HB}\xspace}

%\newcommand{\Mod}{\textit{Mod}\xspace}

%\newcommand{\clc}{\textit{clc}\xspace}



\newcommand{\mcsar}{MCS_{\T}^{AR}\xspace}
\newcommand{\mcsiar}{MCS_{\T}^{IAR}\xspace}
\newcommand{\mcscar}{MCS_{\T}^{CAR}\xspace}
\newcommand{\mcsicar}{MCS_{\T}^{ICAR}\xspace}
\newcommand{\mcsx}{MCS_{\T}^{X}\xspace}

\newcommand{\carrepabox}{\textit{CA-rep}\xspace}
%% esempi KR 2012-LS
\newcommand{\oar}{OA\xspace}
\newcommand{\cox}{CX\xspace}
\newcommand{\crew}{CR\xspace}
\newcommand{\mof}{mf\xspace}
\newcommand{\fb}{fb\xspace}
\newcommand{\rtm}{RTM\xspace}
\newcommand{\ch}{CH\xspace}
\newcommand{\ath}{ATH\xspace}

%%% MACROS sezione 4


\newcommand{\elabel}{\ell}
\newcommand{\colorability}{\mathit{col}}

%\newcommand{\ar}{\mathit{AR}\xspace}
%\newcommand{\iar}{\mathit{IAR}\xspace}
%\newcommand{\cas}{\mathit{CA}\xspace}
%\newcommand{\car}{\mathit{CAR}\xspace}
\newcommand{\carepair}{\mathit{CA}\rm{-repair}\xspace}
%\newcommand{\icar}{\mathit{ICAR}\xspace}

\newcommand{\modelsar}{\models_{\ar}}
\newcommand{\modelsiar}{\models_{\iar}}
\newcommand{\modelscar}{\models_{\car}}
\newcommand{\modelsicar}{\models_{\icar}}

\newcommand{\ia}{\alpha}
\newcommand{\Del}{\D}
\newcommand{\computeiarrepair}{\textit{Compute-IAR-Repair}}
\newcommand{\computeicarrepair}{\textit{Compute-ICAR-Repair}}

\newcommand{\CL}{\mathit{Cl}}
\newcommand{\CR}{\mathit{Cr}}
\newcommand{\QL}{\mathit{Ql}}
\newcommand{\QR}{\mathit{Qr}}
\newcommand{\VL}{\mathit{Vl}}
\newcommand{\VR}{\mathit{Vr}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% SAVO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Ontology-based Information Systems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\ois}{\textsf{OIS}\xspace}
\newcommand{\obdm}{\textsf{ODIS}\xspace}
\newcommand{\ois}{\textsf{OIS}\xspace}
\newcommand{\sois}{\textsf{SOIS}\xspace}
\newcommand{\odis}{\textsf{ODIS}\xspace}
\newcommand{\sot}{SOT\xspace}

\newcommand{\Tinc}{\T_{inc}}
\newcommand{\Ttype}{\T_{type}}
\newcommand{\Tdisj}{\T_{disj}}
\newcommand{\Tfunct}{\T_{funct}}
\newcommand{\Tid}{\T_{id}}
\newcommand{\Tden}{\T_{den}}

\newcommand{\Alphabet}{\Gamma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Inconsistency tolerant Semantics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\arrep}{\textit{AR-Set}\xspace}
\newcommand{\armod}{\textit{Mod}_{AR}\xspace}
\newcommand{\iarrep}{\textit{IAR-Set}\xspace}
\newcommand{\iarmod}{\textit{Mod}_{IAR}\xspace}
\newcommand{\carrep}{\textit{CAR-Set}\xspace}
\newcommand{\carmod}{\textit{Mod}_{CAR}\xspace}
\newcommand{\icarrep}{\textit{ICA-Rep}\xspace}
\newcommand{\icarmod}{\textit{Mod}_{ICAR}\xspace}
\newcommand{\armodels}{\models_\textit{AR}\xspace}
\newcommand{\carmodels}{\models_\textit{CAR}\xspace}
\newcommand{\iarmodels}{\models_\textit{IAR}\xspace}
\newcommand{\icarmodels}{\models_\textit{ICAR}\xspace}
\newcommand{\car}{\textit{CA}\xspace}
\newcommand{\ar}{\textit{A}\xspace}
\newcommand{\iar}{\textit{IA}\xspace}
\newcommand{\icar}{\textit{ICA}\xspace}
\newcommand{\CAR}{\textit{CAR}\xspace}
\newcommand{\AR}{\textit{AR}\xspace}
\newcommand{\IAR}{\textit{IAR}\xspace}
\newcommand{\ICAR}{\textit{ICAR}\xspace}

%%%%%% consistent update
\newcommand{\ComputeInsertion}{\textsf{ComputeInsertion}}
\newcommand{\ComputeDeletion}{\textsf{ComputeDeletion}}
\newcommand{\IncSets}{\textsf{InconsistentSets}}
\newcommand{\delete}{\textsf{Delete}}

%%%%%% inconsistenty-tolerant query answering
\newcommand{\NaiveComputeAnswersar}{\textsf{NaiveComputeAnswers}_{AR}}
\newcommand{\NaiveComputeAnswerscar}{\textsf{NaiveComputeAnswers}_{CAR}}
\newcommand{\NaiveComputeAnswersiar}{\textsf{NaiveComputeAnswers}_{IAR}}
\newcommand{\NaiveComputeAnswersicar}{\textsf{NaiveComputeAnswers}_{ICAR}}
\newcommand{\facts}{\textsf{facts}}
\newcommand{\naiveupdateicar}{\textsf{NaiveComputeUpdate}_{ICAR}}
\newcommand{\computearrep}{\textsf{ComputeARSet}}
\newcommand{\computecarrep}{\textsf{ComputeCARSet}}
\newcommand{\computeiarrep}{\textsf{ComputeIARSet}}
\newcommand{\computeicarrep}{\textsf{ComputeICARSet}}
\newcommand{\computeclc}{\textsf{ComputeCLC}}
\newcommand{\images}{\textsf{images}}
\newcommand{\answericar}{\textsf{ComputeAnswer}_{ICAR}}
\newcommand{\updateicar}{\textsf{ComputeUpdate}_{ICAR}}
%\newcommand{\MinIncSets}{\textsf{MinIncSets}}
\newcommand{\answerDA}{\textsf{Answer}_{DA}}
\newcommand{\answer}{\textsf{Answer}}
\newcommand{\clash}[1]{#1\text{-}clash}
\newcommand{\ca}{\textit{CA}\xspace}
\newcommand{\insop}{\oplus^\T_\cap} %% \ins{\K}{F} inserimento di F in K
\newcommand{\dellop}{\ominus^\T_\cap} %% \del{\K}{F} cancellazione di F da K
\newcommand{\ins}[2]{#1 \insop #2} %% \ins{\K}{F} inserimento di F in K
\newcommand{\insf}[1]{#1 \insop F} %% \insf{\K} inserimento di F in K
\newcommand{\dell}[2]{#1 \dellop #2} %% \del{\K}{F} cancellazione di F da K
\newcommand{\dellf}[1]{#1 \dellop F} %% \delf{\K} cancellazione di F da K
\newcommand{\insopcar}{\oplus^\T_{CAR}} %% \ins{\K}{F} inserimento di F in K
\newcommand{\dellopcar}{\ominus^\T_{CAR}} %% \del{\K}{F} cancellazione di F da K
\newcommand{\inscar}[2]{#1 \insopcar #2} %% \ins{\K}{F} inserimento di F in K
\newcommand{\insfcar}[1]{#1 \insopcar F} %% \insf{\K} inserimento di F in K
\newcommand{\dellcar}[2]{#1 \dellopcar #2} %% \del{\K}{F} cancellazione di F da K
\newcommand{\dellfcar}[1]{#1 \dellopcar F} %% \delf{\K} cancellazione di F da K
\newcommand{\clos}[2]{\textsf{cl}_{#1}(#2)}
\newcommand{\closl}[3]{\textsf{cl}^{#1}_{#2}(#3)}
\newcommand{\Mod}[1]{\mathit{Mod}{(#1)}}
\newcommand{\clc}[1]{\textsf{clc}_{\T}(#1)}
\newcommand{\cl}[1]{\textsf{cl}_{\T}(#1)}
\newcommand{\clt}[1]{\textsf{cl}(#1)}
\newcommand{\TRUE}{\mathit{True}}
\newcommand{\FALSE}{\mathit{False}}
\newcommand{\unsat}{\mathit{Unsat}}



\newcommand{\person}{\textsf{Person}}
\newcommand{\man}{\textsf{Man}}
\newcommand{\woman}{\textsf{Woman}}
\newcommand{\male}{\textsf{Male}}
\newcommand{\female}{\textsf{Female}}
\newcommand{\young}{\textsf{Young}}
\newcommand{\adult}{\textsf{Adult}}
\newcommand{\kid}{\textsf{Kid}}
\newcommand{\hasfather}{\textsf{hasFather}}
\newcommand{\animal}{\textsf{Animal}}
\newcommand{\taylor}{taylor}
\newcommand{\sam}{sam}
\newcommand{\tom}{tom}
\newcommand{\bill}{bill}
\newcommand{\hasparent}{\textsf{hasParent}}


\newcommand{\id}[2]{(\mathsf{id}\; #1\; #2)}
%\newcommand{\val}[1]{\mathit{val}(#1)}
\newcommand{\test}[1]{#1?}
\newcommand{\match}{\mathit{Match}}
\newcommand{\homeTeam}{\mathit{homeTeam}}
\newcommand{\visitorTeam}{\mathit{visitorTeam}}
\newcommand{\playedMatch}{\mathit{playedMatch}}
\newcommand{\sysubset}[2]{#1 \prec_{\Rn} #2}
\newcommand{\Rn}{Rn}
\newcommand{\suba}{\sigma_{\A}\xspace}
\newcommand{\MinIncSet}{\mathit{MinIncSet}}
\newcommand{\IncRewr}{\mathit{IncRewr}}
\newcommand{\IncRewrUCQ}{\mathit{IncRewrUCQ}}
%%\renewcommand{\unify}{\textsf{saturateInequalities}}
\newcommand{\unify}{\textsf{Saturate}}
\newcommand{\compset}{\mathit{CompSet}}
\newcommand{\mvset}{minIncSets\xspace}
\newcommand{\con}{contr\xspace}
\newcommand{\satq}{\textsf{unsatQueries}}
\newcommand{\inQueries}{\textsf{InQueries}\xspace}
\newcommand{\mini}{\textsf{Min}\xspace}
%%\newcommand{\IncSets}{\textsf{witness}\xspace}
\newcommand{\minsatq}{\textsf{minUnsatQueries}\xspace}
\newcommand{\satisfiableden}{\textsf{Satisfiable}_{DA}}
\newcommand{\satisfiable}{\textsf{Satisfiable}}

\newcommand{\IncSng}{\mathit{IncSng}^{\T}}
\newcommand{\ConsAtom}{\mathit{ConsAtom}}
\newcommand{\ConsAtomSet}{\mathit{ConsAtomSet}}
\newcommand{\qunsat}{\Q^{unsat}_{\T}\xspace}
\newcommand{\qsat}{\Q_{str}\xspace}
\newcommand{\qmin}{\Q^{min}_{\T}\xspace}
\newcommand{\clnt}[1]{\mathit{cln}(#1)}
\newcommand{\qsingle}{\Q^{singleton}_{\T}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\digquonto}{DIG-\textsc{QuOnto}\xspace}
\newcommand{\protege}{Prot\'eg\'e\xspace}

\newcommand{\val}[1]{\mathit{val}(#1)}
\newcommand{\cert}[2]{\mathit{cert}(#1,#2)}
\newcommand{\sem}[2]{\mathit{sem}_{#1}(#2)}
\newcommand{\IDC}{\T_{\mathit{id}}}
\newcommand{\GammaVO}{\Gamma_{\mathit{VO}}}
\newcommand{\vc}{\vec{c}}
\newcommand{\chasei}[1]{\mathit{chase}_{#1}(\O)}
\newcommand{\can}[1][\K]{\mathit{can}(#1)}
\newcommand{\cani}[1]{\mathit{can}_{#1}(\O)}
\newcommand{\img}{\G}
\newcommand{\qv}[1]{\texttt{#1}}
\newcommand{\qo}[1]{\textsl{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\pse}{(\Leftarrow)}
%\newcommand{\psolose}{(\Rightarrow)}
\newcommand{\ifdirection}{(\Leftarrow)}
\newcommand{\onlyifdirection}{(\Rightarrow)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% MACROS EXAMPLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% MACROS esempi
\newcommand{\DR}{\textsf{Driver}}
%%\newcommand{\CR}{\textsf{Car}}
\newcommand{\TM}{\textsf{TeamMember}}
\newcommand{\MC}{\textsf{Mechanic}}
\newcommand{\drives}{\textsf{drives}}
\newcommand{\FOT}{FT}

%% MACROS RR 2011
\newcommand{\notincoherent}{\mathit{ConsAtom}}
\newcommand{\disjointattrdomains}{\mathit{DisjAttrDom}}
\newcommand{\disjointconceptnames}{\mathit{DisjConcepts}}
\newcommand{\disjointroledomains}{\mathit{DisjRoleDom}}
\newcommand{\disjointroleranges}{\mathit{DisjRoleRan}}
\newcommand{\disjointrolenames}{\mathit{DisjRoles}}
\newcommand{\disjointinverseroles}{\mathit{DisjInvRoles}}
\newcommand{\disjointattributes}{\mathit{DisjAttributes}}
\newcommand{\notdisjclash}{\mathit{NotDisjClash}}
\newcommand{\notfunctclash}{\mathit{NotFunctClash}}
\newcommand{\notclash}{\mathit{NotClash}}
\newcommand{\iarincrewriting}{\textit{IncRewriting}_{\iar}}
\newcommand{\iarincrewritingUCQ}{\textit{IncRewritingUCQ}_{\iar}}
\newcommand{\icarincrewritingUCQ}{\textit{IncRewritingUCQ}_{\icar}}
\newcommand{\icarincrewriting}{\textit{IncRewriting}_{\icar}}
\newcommand{\iarrewriting}{\textit{PerfectRef}_{\iar}}
\newcommand{\icarrewriting}{\textit{PerfectRef}_{\icar}}
\newcommand{\aczero}{\mathit{AC}^0}
\newcommand{\pidue}{\Pi^p_2}

%%IJCAI 2017


\newcommand{\add}[1]{\textsf{i}(#1)}
\newcommand{\del}[1]{\textsf{d}(#1)}
\newcommand{\Const}{\mathit{Const}}


%%%examples
\newcommand{\emp}{\textit{employee}\xspace}
\newcommand{\mgr}{\textit{manager}\xspace}
\newcommand{\worksfor}{\textit{WORKS-FOR}\xspace}
\newcommand{\tempemp}{\textit{tempEmp}\xspace}
\newcommand{\until}{\textsf{until}\xspace}
\newcommand{\proj}{\textit{project}\xspace}
\newcommand{\manages}{\textit{MANAGES}\xspace}
\newcommand{\xsddate}{\texttt{xsd:date}\xspace}
\newcommand{\palm}{\textbf{Palm}\xspace}
\newcommand{\lenz}{\textbf{White}\xspace}
\newcommand{\projquonto}{\textbf{DIS-1212}\xspace}
\newcommand{\projtones}{\textbf{FP6-7603}\xspace}
\newcommand{\projname}{\mathsf{ProjName}\xspace}
\newcommand{\pname}{\mathsf{PersName}\xspace}
\newcommand{\xsdstring}{\texttt{xsd:string}\xspace}
%\newcommand{\pid}{\textbf{project}\xspace}
\newcommand{\projectbf}{\textbf{proj}\xspace}
%\newcommand{\personSSN}{\textbf{person}\xspace}
\newcommand{\personbf}{\textbf{pers}\xspace}
%\newcommand{\oid}{\textbf{manager}\xspace}
\newcommand{\managerbf}{\textbf{mgr}\xspace}
%\newcommand{\person}{\textit{person}\xspace}
\newcommand{\term}{\textsl{25-09-05}\xspace}
\newcommand{\quontoname}{\textsl{QuOnto}\xspace}
\newcommand{\tonesname}{\textsl{Tones}\xspace}
\newcommand{\lenznid}{\textsl{X11}\xspace}
\newcommand{\lenzname}{\textsl{White}\xspace}
\newcommand{\nardnid}{\textsl{X12}\xspace}
\newcommand{\nardname}{\textsl{Black}\xspace}
\newcommand{\ssna}{\textsl{20903}\xspace}
\newcommand{\salarya}{\textsl{1000}\xspace}
\newcommand{\namea}{\textsl{Rossi}\xspace}
\newcommand{\nameb}{\textsl{White}\xspace}
\newcommand{\ssnb}{\textsl{55577}\xspace}
\newcommand{\ssnc}{\textsl{29767}\xspace}

%%%%%ESEMPIO RETE DI ACCESSO
\newcommand{\device}{\textit{Device}\xspace}
\newcommand{\port}{\textit{Port}\xspace}
\newcommand{\portin}{\textit{PortIn}\xspace}
\newcommand{\portout}{\textit{PortOut}\xspace}
\newcommand{\connectedTo}{\textit{connectedTo}\xspace}
\newcommand{\of}{\textit{of}\xspace}
\newcommand{\num}{\textit{number}\xspace}


%%%%%%ESEMPIO AREOPORTI
\newcommand{\flight}{\textsf{Flight}\xspace}
\newcommand{\arrival}{\textsf{arrival}\xspace}
\newcommand{\departure}{\textsf{departure}\xspace}
\newcommand{\airport}{\textsf{Airport}\xspace}
\newcommand{\company}{\textsf{Company}\xspace}
\newcommand{\city}{\textsf{City}\xspace}
\newcommand{\locatedIn}{\textsf{locatedIn}\xspace}
\newcommand{\belongsTo}{\textsf{belongsTo}\xspace}
\newcommand{\name}{\textit{name}\xspace}
%\newcommand{\code}{\textit{code}\xspace}
\newcommand{\xsdinteger}{\texttt{xsd:integer}\xspace}


\newcommand{\red}{red\xspace}
\newcommand{\blue}{blue\xspace}
\newcommand{\green}{green\xspace}
\newcommand{\brown}{brown\xspace}
\newcommand{\Color}{\textsf{Color}\xspace}
\newcommand{\CColor}{\textsf{CoolColor}\xspace}
\newcommand{\WColor}{\textsf{WarmColor}\xspace}

\newcommand{\son}{\textsf{Son}\xspace}
\newcommand{\husband}{\textsf{Husband}\xspace}
%\newcommand{\man}{\textsf{Man}\xspace}
%\newcommand{\woman}{\textsf{Woman}\xspace}
\newcommand{\conjset}{conj\text{-}set}

%%% KR'08
\newcommand{\Ofbc}{\O_{\mathit{fbc}}}
\newcommand{\Tfbc}{\T_{\mathit{fbc}}}
\newcommand{\Afbc}{\A_{\mathit{fbc}}}
\newcommand{\League}{\textit{League}}
\newcommand{\Nation}{\textit{Nation}}
\newcommand{\Team}{\textit{Team}}
\newcommand{\Round}{\textit{Round}}
\newcommand{\Match}{\textit{Match}}
\newcommand{\PlayedMatch}{\textit{PlayedMatch}}
\newcommand{\ScheduledMatch}{\textit{ScheduledMatch}}
\newcommand{\OF}{\textit{OF}}
\newcommand{\BELONGSTO}{\textit{BELONGS-TO}}
\newcommand{\PLAYEDIN}{\textit{PLAYED-IN}}
\newcommand{\NEXT}{\textit{NEXT}}
\newcommand{\HOST}{\textit{HOST}}
\newcommand{\HOME}{\textit{HOME}}
\newcommand{\yearE}{\mathbf{year}}
\newcommand{\code}{\mathbf{code}}
\newcommand{\dateE}{\mathbf{date}}
\newcommand{\homeGoals}{\mathbf{homeGoals}}
\newcommand{\hostGoals}{\mathbf{hostGoals}}
\newcommand{\xsdnonneg}{\texttt{xsd:nonNegativeInteger}}
\newcommand{\xsdint}{\texttt{xsd:positiveInteger}}

%%%%MACRO ESWC-12-LSS
\newcommand{\topp}{\top_P}
\newcommand{\topa}{\top_A}
\newcommand{\botc}{\bot_C}
\newcommand{\botp}{\bot_P}
\newcommand{\bota}{\bot_A}

\newcommand{\cla}{\beta\text{-}cl(\T)}
\newcommand{\clat}{cl(\T)}
\newcommand{\pse}{(\Leftarrow)}
\newcommand{\psolose}{(\Rightarrow)}
\newcommand{\pred}{\textsf{predecessors}}

\newcommand{\Cu}{\Phi_{\T}}
\newcommand{\Cd}{\Omega_{\T}}
\newcommand{\Gstar}{\G^*_{\T}}
\newcommand{\Estar}{\E^*}
\newcommand{\alphae}{\alpha(\Estar)}
\newcommand{\computeNeg}{\textsf{computeNeg}}


%%% MACROS esempi
%\newcommand{\DR}{\textsf{Driver}}
%\newcommand{\CR}{\textsf{Car}}
%\newcommand{\TM}{\textsf{TeamMember}}
%\newcommand{\MC}{\textsf{Mechanic}}
%\newcommand{\drives}{\textsf{drives}}


==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%% notes and todos

\ifdraft
\newcounter{todocntr}
\newenvironment{todoenv}
  {\addtocounter{todocntr}{1}\par\bigskip\noindent
   \color{blue}\fbox{\thetodocntr}\hspace*{\fill}~\bf
   \begin{minipage}[t]{0.95\linewidth}}
  {\end{minipage}\hspace*{\fill}\bigskip}
%\newcommand{\todo}[1]{\begin{todoenv}{#1}\end{todoenv}}
\newcommand{\td}[1]{\noindent{\color{red}\framebox[\linewidth]{\parbox{0.95\linewidth}{\bf #1}}}}
\makeatletter
\if@twocolumn
  \newcommand{\nb}[1]{{\color{red}\it\par[[#1]]\par}}
\else
  \setlength{\marginparwidth}{20mm}
  \newcommand{\nb}[1]{\textcolor{red}{\bf!}%
   \marginpar[\parbox{20mm}{\scriptsize\textcolor{red}{\raggedleft #1}}]%
   {\parbox{20mm}{\scriptsize\textcolor{red}{\raggedright #1}}}}
\fi
\makeatother
\else
\newcommand{\td}[1]{}
\newcommand{\nb}[1]{}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%% Environments

%\usepackage{amsthm}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}

%\theoremstyle{definition}

\newtheorem{exampleAux}{Example}
%\newenvironment{example}{\begin{exampleAux}\rm}{\end{exampleAux}\par\smallskip}
%\newtheorem{example}{Example}

%\newenvironment{proof}{\noindent\textsl{Proof.\ }}{\qed\par\smallskip}
 \newenvironment{proofsk}{\noindent\textsl{Proof (sketch).\ }}{\qed}

\def\qed{\hfill{\qedboxempty}} % qed with empty box
\def\qedboxempty{\vbox{\hrule\hbox{\vrule\kern3pt
\vbox{\kern3pt\kern3pt}\kern3pt\vrule}\hrule}}

\def\qedfull{\hfill{\qedboxfull}}
\def\qedboxfull{\vrule height 5pt width 5pt depth 0pt}

%%%%%%%%%%%%%%%%%%%%%%%%%% General Math

\newcommand{\A}{\mathcal{A}} \newcommand{\B}{\mathcal{B}}
\newcommand{\C}{\mathcal{C}} \newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathcal{E}} \newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}} \renewcommand{\H}{\mathcal{H}}
\newcommand{\I}{\mathcal{I}} \newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}} \renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}} \newcommand{\N}{\mathcal{N}}
\renewcommand{\O}{\mathcal{O}} \renewcommand{\P}{P}
\newcommand{\Q}{\mathcal{Q}} \newcommand{\R}{\mathcal{R}}
\renewcommand{\S}{\mathcal{S}} \newcommand{\T}{\mathcal{T}}
\newcommand{\U}{\mathcal{U}} \newcommand{\V}{\mathcal{V}}
\newcommand{\W}{\mathcal{W}} \newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}} \newcommand{\Z}{\mathcal{Z}}

\newcommand{\mf}{\mathfrak}

%%%%%%%%%%%%%%%%%%%%%%%%%% Abbreviations

\newcommand{\setone}[2][1]{\set{#1\cld #2}}
\newcommand{\eset}{\emptyset}
%%\newcommand{\col}{\colon}
\newcommand{\ol}[1]{\overline{#1}}                % overline
%\newcommand{\ul}[1]{\underline{#1}}               % underline
\newcommand{\uls}[1]{\underline{\raisebox{0pt}[0pt][0.45ex]{}#1}}

%% ul with space between text and line

\newcommand{\ra}{\rightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Lra}{\Leftrightarrow}
\newcommand{\lora}{\longrightarrow}
\newcommand{\Lora}{\Longrightarrow}
\newcommand{\lola}{\longleftarrow}
\newcommand{\Lola}{\Longleftarrow}
\newcommand{\lolra}{\longleftrightarrow}
\newcommand{\Lolra}{\Longleftrightarrow}
\newcommand{\ua}{\uparrow}
\newcommand{\Ua}{\Uparrow}
\newcommand{\da}{\downarrow}
\newcommand{\Da}{\Downarrow}
\newcommand{\uda}{\updownarrow}
\newcommand{\Uda}{\Updownarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%% Relations

\newcommand{\incl}{\subseteq}
\newcommand{\imp}{\rightarrow}
%%\newcommand{\deq}{\doteq}
\newcommand{\dleq}{\dot{\leq}}                   % dotted less equal

%%%%%%%%%%%%%%%%%%%%%%%%%% Spaces

%\newcommand{\per}{\mbox{\bf .}}                  % period

\newcommand{\cld}{,\ldots,}                      % ,...,
\newcommand{\ld}[1]{#1 \ldots #1}                 % #1 ... #1
\newcommand{\cd}[1]{#1 \cdots #1}                 % #1 ... #1
\newcommand{\lds}[1]{\, #1 \; \ldots \; #1 \,}    % _#1_..._#1_
\newcommand{\cds}[1]{\, #1 \; \cdots \; #1 \,}    % _#1_..._#1_

%%%%%%%%%%%%%%%%%%%%%%%%%% Delimiters

\newcommand{\set}[1]{\{#1\}}                      % set
%\newcommand{\Set}[1]{\left\{#1\right\}}
%%\newcommand{\bigset}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\bigmid}{\Big|}
\newcommand{\card}[1]{|{#1}|}                     % cardinality of a set
\newcommand{\Card}[1]{\left| #1\right|}
\newcommand{\cards}[1]{\sharp #1}
\newcommand{\tup}[1]{(#1)}            % tuple
\newcommand{\Tup}[1]{\left\langle #1\right\rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\myi}{\emph{(i)}\xspace}
\newcommand{\myii}{\emph{(ii)}\xspace}
\newcommand{\myiii}{\emph{(iii)}\xspace}
\newcommand{\myiv}{\emph{(iv)}\xspace}
\newcommand{\myv}{\emph{(v)}\xspace}
\newcommand{\myvi}{\emph{(vi)}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%% DL specific commands

\newcommand{\PTIME}{\textsc{PTime}\xspace}
\newcommand{\EXPTIME}{\textsc{ExpTime}\xspace}
\newcommand{\PSPACE}{\textsc{Pspace}\xspace}
\newcommand{\ACz}{AC\ensuremath{^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%% Interpretation

\newcommand{\inter}[1][\I]{(\dom[#1],\Int[#1]{\cdot})}   % (dom^I,.^I)

\newcommand{\dom}[1][\I]{\Delta^{#1}}  % delta^I (domain of interpretation \I)
\newcommand{\Int}[2][\I]{#2^{#1}}      % #2^I    (interpretation function)
\newcommand{\INT}[2][\I]{(#2)^{#1}}    % (#2)^I  (interpretation function)

%%%%%%%%%%%%%%%%%%%%%%%%%% Basic Concept forming operators

\newcommand{\AND}{\sqcap}
\newcommand{\OR}{\sqcup}
\newcommand{\NOT}{\neg}
\newcommand{\ALL}[2]{\forall #1 \per #2}
\newcommand{\SOME}[2]{\exists #1 \per #2}
\newcommand{\SOMET}[1]{\exists #1}
\newcommand{\ALLRC}{\ALL{R}{C}}
\newcommand{\SOMERC}{\SOME{R}{C}}
\newcommand{\SOMERT}{\SOMET{R}}
\newcommand{\ATLEAST}[2]{(\geq #1 \, #2)}
\newcommand{\ATMOST}[2]{(\leq #1 \, #2)}
\newcommand{\EXACTLY}[2]{(= #1 \, #2)}
\newcommand{\INV}[1]{#1^{-}}

%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\BOX}[1]{ [\!-\!] #1}
\newcommand{\DIAM}[1]{\langle \!-\!\rangle #1}
%\newcommand{\BOX}[2]{ [{#1}] #2}
%\newcommand{\DIAM}[2]{\langle {#1} \rangle #2}

\newcommand{\QATMOST}[3]{(\leq #1\; \DIAM{#2}{#3})}
%%\newcommand{\QATLEAST}[3]{(\geq #1\, #2 \per #3)}

\newcommand{\ISA}{\sqsubseteq}
\newcommand{\EQU}{\equiv}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro and personal command
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%\newcommand{\limp}{\rightarrow}
\newcommand{\limp}{\rightarrow}
\newcommand{\lequiv}{\leftrightarrow}
\newcommand{\conc}{\mathord{\cdot}}

%%%%%%%%%%% Mu-Calculus Interpretation: \mf{A}, \V

\newcommand{\MOD}[1]{(#1)^{\mf{}}}
\newcommand{\Moda}[1]{#1_{\V}^{\mf{}}}     % argument_{\V}^\mf{A} % Giuseppe
                                        % interp. and assign. fun.
\newcommand{\Modax}[2]{#1_{\V #2}^\mf{A}} % argument_{\V}^\mf{A} % Giuseppe
                                        % interp. and modif. assign. fun.
%\newcommand{\MODA}[1]{(#1)_{\V}^\mf{A}}   % (argument)_{\V}^\mf{A} % Giuseppe
%                                        % interp. and assign. fun.
%\newcommand{\MODAX}[2]{(#1)_{\V #2}^\mf{A}} % (argument)_{\V.}^\mf{A} % Giuseppe
%                                        % interp. and
%                                        % modif. assign. fun.

\newcommand{\MODA}[1]{(#1)_{\vfo,\vso}^{\mf{}}}   % (argument)_{\V}^\mf{A} %
                                % Giuseppe modified by Marco
                                        % interp. and assign. fun.

\newcommand{\MODAfirst}[1]{(#1)_{\vfo}^\mf{A}}   % (argument)_{\V}^\mf{A} %
                                % Giuseppe modified by Marco
                                        % interp. and assign. fun.


\newcommand{\MODAX}[2]{(#1)_{\vfo #2,\vso}^{\mf{}}}   % (argument)_{\V}^\mf{A} %
                                % Giuseppe modified by Marco
                                        % interp. and assign. fun.

\newcommand{\MODAZ}[2]{(#1)_{\vfo,\vso #2}^{\mf{}}}   % (argument)_{\V}^\mf{A} %
                                % Giuseppe modified by Marco
                                        % interp. and assign. fun.

\newcommand{\MODATX}[3]{(#1)^{#2}_{#3}}
\newcommand{\Modat}[2]{#1_{\V}^{#2}}     % argument_{\V}^\mf{A}
                                        % interp. and assign. fun.
\newcommand{\MODAT}[2]{(#1)_{\V}^{#2}}   % (argument)_{\V}^\mf{A}
                                        % interp. and assign. fun.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}

\newcommand{\dllite}{\textit{DL-Lite}\xspace}
\newcommand{\dllitef}{\textit{DL-Lite}\ensuremath{_{\mathcal{F}}}\xspace}
\newcommand{\dlliter}{\textit{DL-Lite}\ensuremath{_{\mathcal{R}}}\xspace}
\newcommand{\dllitea}{\textit{DL-Lite}\ensuremath{_{\mathcal{A}}}\xspace}
%%\newcommand{\dllitenouna}{\textit{DL-Lite}\ensuremath{_{\mathcal{A}}^{\lnot\textsc{una}}}\xspace}
\newcommand{\dllitenouna}{\textit{DL-Lite}\ensuremath{_\textsc{nu}}\xspace}

\newcommand{\ALCQI}{\ensuremath{\mathcal{ALCQI}}}


\newcommand{\cert}[1]{\mathit{cert}(#1)}
\newcommand{\ans}[2][]{\mathit{ans}_{#1}(#2)}
\newcommand{\rew}[1]{\mathit{rew}(#1)}
\newcommand{\goto}[1][\mf{A}]{\mathrel{\Ra_{#1}}}

\newcommand{\conj}{\mathit{conj}}

\newcommand{\homom}[4][\C]{#3 \mathrel{\ra^{#1}_{#2}} #4}
\newcommand{\map}[2]{#1 \rightsquigarrow #2}
\newcommand{\carule}[2]{#1 \mapsto #2}

\renewcommand{\A}{A}
\renewcommand{\T}{T}
\renewcommand{\R}{R}
%%\renewcommand{\C}{C} %%%GGG altrimenti si confonde con i concetti

\newcommand{\Amax}{\A_{\mathit{max}}}

\newcommand{\ex}[1]{\mathsf{#1}}
\newcommand{\actex}[1]{\mathsf{#1}}

\newcommand{\const}[1]{\C_{#1}}

\newcommand{\Act}{\mathit{Act}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% For IJCAI 2013

\newcommand{\dlds}{Description Logic based Dynamic System\xspace}
\newcommand{\kbds}{\dlds}

\newcommand{\kgds}{DL based 2GS\xspace}
\newcommand{\kds}{DLDS\xspace}
\newcommand{\kgs}{KGS\xspace}

\newcommand{\kdsys}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\kgsys}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\f}{\tau}
\newcommand{\aboxt}{\mathcal{A}_\T}
\newcommand{\bij}{h}
\newcommand{\bijdomain}{S_1}
\newcommand{\bijrange}{S_2}

\newcommand{\mymu}{\ensuremath{\mu\mathit{DL}_p}\xspace}
\newcommand{\muADLp}{\ensuremath{\mu\mathit{ADL}_p}\xspace}

\newcommand{\univ}{\ensuremath{\Delta}\xspace}
\newcommand{\free}[1]{\textsc{free}(#1)}
\newcommand{\pmap}{m}
\newcommand{\pset}{\P}
\newcommand{\psel}{\pi}
\newcommand{\psubset}{D_\P}
\newcommand{\actset}{\Gamma}
\newcommand{\system}{s}
\newcommand{\env}{e}
\newcommand{\agent}{a}

\newcommand{\Turn}{\mathsf{Turn}}
\newcommand{\force}{\ensuremath{[\!\langle\!-\!\rangle\!]}}
\newcommand{\forces}{\force_s}
\newcommand{\forcew}{\force_w}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% For KR 2012
\newcommand{\funct}[1]{(\ex{funct}~#1)}
\newcommand{\idconstr}[2]{(\ex{id}~#1~#2)}
\newcommand{\adom}[1]{\textsc{adom}(#1)}
\newcommand{\idom}[1]{\textsc{idom}(#1)}

\newcommand{\eq}[2]{#1 = #2}
\newcommand{\Eq}[1]{\textsc{eq}(#1)}
\newcommand{\DO}[1]{\textsc{do}(#1)}

\newcommand{\Ans}[2][]{\textsc{ans}_{#1}(#2)}
\newcommand{\arAns}[2][]{\textsc{ar-ans}_{#1}(#2)}

\newcommand{\Tuna}{T^{\textsc{una}}}
\newcommand{\Tnouna}{T^{\st{\textsc{una}}}}

\newcommand{\abox}{\mathit{abox}}
%%\renewcommand{\do}{do}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PODS2012
%------------------------------------------------------------- Domain
\newcommand{\CONST}{C}
%\newcommand{\adom}[1]{\textsc{adom}(#1)}

\newcommand{\FUNC}{\ensuremath{\F}\xspace}   % Set of function names
\newcommand{\HERBAND}{\HERBRAND}
\newcommand{\HERBRAND}{\ensuremath{\mathbb{U}}\xspace}
 % Herbrand universe
\newcommand{\PART}[1]{\ensuremath{P^{#1}}}   % Partitioning of a given set

%------------------------------------------- Data Layer
\newcommand{\dl}{\ensuremath{\D}\xspace}
\newcommand{\schema}{\ensuremath{\R}\xspace}
%\newcommand{\schema}{\bsy{R}}
\newcommand{\idb}{\ensuremath{\I_0}\xspace}
%------------------------------------------- Process Layer
\newcommand{\pl}{\ensuremath{\P}\xspace}
\newcommand{\aset}{\ensuremath{\A}\xspace}
\newcommand{\rset}{\ensuremath{\varrho}\xspace}
\newcommand{\pos}[1]{\ensuremath{#1^+}\xspace}

\newcommand{\sys}{\ensuremath{\S}\xspace}
\newcommand{\dcds}{\mbox{DCDS}\xspace}
\newcommand{\rexec}[1]{\textsc{exec}_{#1}\xspace}
\newcommand{\sexec}[1]{\textsc{s-exec}_{#1}\xspace}

%------------------------------------------- Properties

\newcommand{\mulg}{\mulgq}
\newcommand{\muladom}{\ensuremath{\muL_{A}}\xspace}
\newcommand{\mulpers}{\ensuremath{\muL_{P}}\xspace}
\newcommand{\hmadom}{\ensuremath{\L_{A}}\xspace}
\newcommand{\hmpers}{\ensuremath{\L_{P}}\xspace}

\newcommand{\hbsim}{\approx}
\newcommand{\pbsim}{\sim}


\newcommand{\inadom}{\ensuremath{\textsc{live}}}

\newcommand{\restrict}[2]{\ensuremath{#1 \vert_{#2}}}

\newcommand{\muL}{\mu\L} % MuL - modal mu calculus - language
\newcommand{\muLclosed}{\muL_{C}}
\newcommand{\muLinitialdomain}{\muL_{{\I_0}}}
\newcommand{\muLguarded}{\muL_{G}}
\newcommand{\hmLguarded}{\L_{G}}
\newcommand{\muLglobal}{\muL_{\forall\exists G}}
%\newcommand{\muLglobal}{\muL_{(\forall,\exists)^*G}}

%------------------------------------------- Artifact System Syntax

\newcommand{\rmap}{\ensuremath{\M}\xspace}
\newcommand{\rmapext}{\ensuremath{\widehat{\M}}\xspace}

\newcommand{\rmapec}{\ensuremath{\rmap}}
   % Interpretation  of skolem terms
%\renewcommand{\terms}[1]{\textsc{terms}(#1)} % terms used in a given
                                % partitioning
\newcommand{\subterms}{\textsc{subTerms}}
\newcommand{\EC}{\ensuremath{\E}}       % Set of equality constraints
\newcommand{\ec}{\textit{ec}}          % An equality constraint.
\newcommand{\history}{\ensuremath{\H}} % History of a artifact system
                                % instance

%----------------------------------------------------------------
\newcommand{\VDO}[4]{\mbox{DO}^V\big(#1,\ #2,\ #3,\ #4\big)}
\newcommand{\RDO}[3]{\mbox{DO}^R\big(#1,\ #2,\ #3\big)}
\newcommand{\SDO}[3]{\mbox{DO}^S\big(#1,\ #2,\ #3\big)}

\newcommand{\VCLOSURE}[3]{\mbox{CLOSURE}^V\big(#1,\ #2,\ #3\big)}
\newcommand{\RCLOSURE}[3]{\mbox{CLOSURE}^R\big(#1,\ #2,\ #3\big)}
\newcommand{\SCLOSURE}[3]{\mbox{CLOSURE}^S\big(#1,\ #2,\ #3\big)}

\newcommand{\VEXECUTE}[3]{\mbox{EXECUTE}_{closed}^V\big(\tup{#1,#2},\ #3\big)}
\newcommand{\REXECUTE}[3]{\mbox{EXECUTE}_{closed}^ R\big(\tup{#1,#2},\ #3\big)}
\newcommand{\SEXECUTE}[3]{\mbox{EXECUTE}_{closed}^S\big(\tup{#1,#2},\ #3\big)}

%-----------------------------------------------------------------

% Next generations of Do, Closure, and Execute:

\newcommand{\merge}{\textsc{merge}}

\newcommand{\doo}[3]{\textsc{do}^{#1}_{#2}(#3)}
\newcommand{\effect}[1]{\textsc{effect}(#1)}
% \do { S | R | V }{CLOSE | OPEND | OPENN} { \I,\P, ... }

\newcommand{\closure}[3]{\textsc{closure}^{#1}_{#2}(#3)}
% \closure { S | R | V }{CLOSE | OPEND | OPENN} { \I,\P, ... }

\newcommand{\sexecute}[3]{\textcolor{red}{\textsc{s-}\execute{#1}{#2}{#3}}\xspace}
\newcommand{\rexecute}[3]{\textcolor{red}{\execute{#1}{#2}{#3}}\xspace}

\newcommand{\execute}[3]{\ensuremath{\textsc{execute}^{#1}_{#2}#3}\xspace}
% \execute { S | R | V }{CLOSE | OPEND | OPENN} { \I,\P, ... }
%------------------------------------------------------------------

\newcommand{\VEXECUTEO}[3]{\mbox{EXECUTE}_{open}^V\big(\tup{#1,#2},\ #3\big)}
\newcommand{\REXECUTEO}[3]{\mbox{EXECUTE}_{open}^R\big(\tup{#1,#2},\ #3\big)}
\newcommand{\SEXECUTEO}[3]{\mbox{EXECUTE}_{open}^S\big(\tup{#1,#2},\ #3\big)}

\newcommand{\RDOC}{\mbox{DO}^R}
\newcommand{\SDOC}{\mbox{DO}^S}

\newcommand{\REXTRC}{\mbox{EXTRACT\_CALLS}}
\newcommand{\REXTRCL}{\mbox{EXTRACT\_CLASSES}}
\newcommand{\RCALLC}{\textsc{serviceCalls}}
\newcommand{\RCOMM}{\textsc{pickCommitment}}
\newcommand{\pickVal}{\textsc{pickValue}}
\newcommand{\callService}{\textsc{callService}}

%-----------------------------------------------------------------

%\newcommand{\PICK}[2]{\mbox{PICK}(#1,\  #2)}
%\newcommand{\transition}[5]{\tup{#2,#3}\mapsto^{#1}\tup{#4,#5}}

\newcommand{\cts}[1]{\Upsilon_#1}
\newcommand{\sts}[1]{\Theta_#1}
\newcommand{\bts}[1]{\Lambda_#1}
\newcommand{\ats}[1]{\bar\Upsilon_#1}

\newcommand{\VT}[2]{\Upsilon^V(#1,#2)}
\newcommand{\RT}[2]{\textcolor{red}{\Upsilon(#2,#1)}}
\newcommand{\ST}[2]{\textcolor{red}{\Upsilon_S(#2,#1)}}
\newcommand{\GT}[2]{\Upsilon(#1,#2)}
%\renewcommand{\mf}[1]{{\Upsilon(\mathcal{#1})}}
\renewcommand{\mf}[1]{\Upsilon_{#1}}
\newcommand{\db}{\mathit{db}}
\newcommand{\rel}[1]{\db(#1)}
\newcommand{\domdb}{\mathit{dom}}

\newcommand{\ISM}[1]{\equiv_{#1}}
\newcommand{\EISM}[1]{\cong_{#1}}
\newcommand{\EMISM}[1]{\unrhd_{#1}}

\newcommand{\DUNION}{\overset{+}{\cup}}

\newcommand{\RI}{\mathfrak{I}^R}

\newcommand{\Prj}[2]{#1|_{#2}}

 \newcommand{\valueof}[1]{\ensuremath{\textsc{value}_{#1}}}
 \newcommand{\nullvalue}{\ensuremath{\chi}}
%%% END

%% Macros by Marco


\newcommand{\realdom}{\ensuremath{\C}\xspace}
\newcommand{\scset}{\ensuremath{\mathbb{SC}}\xspace}

\newcommand{\comp}{\triangleright}
\newcommand{\bcomp}{h}

\newcommand{\UPDATE}{\mbox{UPDATE}}
\newcommand{\EXTRDIS}{\mbox{INFER\_DIS}}

\newcommand{\newskolems}{\textit{NS}}
\newcommand{\DSet}{\D}
\newcommand{\CongClosureS}{\mbox{CONGRUENCE\_CLOSURE}^S}
\newcommand{\domain}[1]{\ensuremath{\textsc{dom}(#1)}\xspace}
\newcommand{\image}[1]{\ensuremath{\textsc{im}(#1)}\xspace}

\newcommand{\embeddedfig}[2]
{
	\begin{minipage}{#2}
		\noindent
		\includegraphics[width=#2]{#1}
	\end{minipage}
}

\newcommand{\wrt}{w.r.t.\ }

\newcommand{\had}[1]{\domain{#1}}%{\ensuremath{\widehat{\C_{#1}}}\xspace}
\newcommand{\hd}[1]{\ensuremath{\Delta_{#1}}\xspace}
\newcommand{\rep}[2]{\ensuremath{\textsc{rep}_{#2}(#1)}}
\newcommand{\repset}[1]{\ensuremath{\textsc{rep}(#1)}}
\newcommand{\repsetc}[1]{\ensuremath{\textsc{rep}_c(#1)}}
\newcommand{\chooserep}[1]{\ensuremath{\textsc{chooseRep}(#1)}}
\newcommand{\phd}[1]{\ensuremath{\textsc{im}_{#1}}}

%\usepackage{color}
%\newcommand{\todo}[1]{\footnote{\scriptsize\textbf{\textcolor{red}{#1}}}}
\newcommand{\tocheck}[1]{\textcolor{red}{#1}}

%\newcommand{\boxdiamond}{\ensuremath{\medbox \hspace{-.62em} \diamond}\xspace}

% \newcommand{\rewritef}[2]{\ensuremath{\textsc{rf}^{#1}_{#2}}}
% \newcommand{\rewritets}[2]{\ensuremath{\textsc{modTS}^{#1}_{#2}}}

\newcommand{\rewritefclosed}{\textsc{rf-cl}}
\newcommand{\rewritetsclosed}{\textsc{tr-cl}}
\newcommand{\rewritefinitial}{\textsc{rf-iad}}
\newcommand{\rewritetsinitial}{\textsc{tr-iad}}
\newcommand{\rewritefguarded}{\textsc{rf-gu}}
\newcommand{\rewritetsguarded}{\textsc{rf-gu}}
\newcommand{\rewritefglobal}{\textsc{rf-gl}}
\newcommand{\rewritemglobal}{\textsc{rmod-gl}}
\newcommand{\rewritetsglobal}{\textsc{tr-gl}}

\newcommand{\statename}{\textsc{sn}}

\newcommand{\someop}{\ensuremath{\circledast}\xspace}
\newcommand{\rewritemodf}{\textsc{rewriteMod}}
\newcommand{\rewritemod}[2]{\ensuremath{\rewritemodf_{#1}\left(#2\right)}}
\newcommand{\rewritequantf}{\textsc{replaceQuant}}
\newcommand{\rewritequant}[2]{\ensuremath{\rewritequantf_{#1}\left(#2\right)}}
\newcommand{\extterm}{t}
\newcommand{\somesymbol}{\circledast}

\newcommand{\abst}[1]{\bar #1}
\newcommand{\globalschema}{\R}

\newcommand{\ientailment}[3]{#1\models #2#3}
\newcommand{\entailment}[4]{#1,#2\models #3#4}
%\renewcommand{\entailment}[4]{#2 \in (#3)^{#1}_{#4}}

\newcommand{\nentailment}[4]{#1,#2\not\models #3#4}
%\renewcommand{\nentailment}[4]{#2 \not\in (#3)^{#1}_{#4}}



%\DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
%\DeclareMathSymbol{\varheart}{\mathalpha}{extraup}{86}
%\DeclareMathSymbol{\vardiamond}{\mathalpha}{extraup}{87}
%\DeclareSymbolFont{lasy}{U}{lasy}{m}{n}
%\DeclareMathSymbol\BlackDiamond{\mathord}{lasy}{"12}
%\DeclareSymbolFont{pxsymbolsC}{U}{pxsyc}{m}{n}
%\SetSymbolFont{pxsymbolsC}{bold}{U}{pxsyc}{bx}{n}
%\DeclareMathSymbol{\Diamondblack}{\mathrel}{pxsymbolsC}{95}
%\DeclareMathSymbol{\Squareblack}{\mathrel}{pxsymbolsC}{4}

%\newcommand{\Diamondblack}{\rotatebox[origin=c]{45}{$\Diamond$}}


%% ------------------------------------- New introduced by Babak

\newcommand{\ASINSTANCE}{\I}
\newcommand{\AINSTANCE}{I}

%%------------------------------------- Texts

\newcommand{\cstate}{\mbox{c-state}\xspace}
\newcommand{\sstate}{\mbox{s-state}\xspace}
\newcommand{\SINSTANCE}{\mbox{s-state}\xspace}
\newcommand{\RINSTANCE}{\mbox{c-state}\xspace}
\newcommand{\VINSTANCE}{\mbox{v-instance}\xspace}
\newcommand{\GINSTANCE}{\mbox{instance}\xspace}

\newcommand{\EISOMORPHIC}{\mbox{e-isomorphic}}


\newcommand{\vfo}{\ensuremath{v}}
\newcommand{\vso}{\ensuremath{V}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Babak

\newcommand{\brem}[1]{{\textcolor{blue}{\small\it [[{#1} --babak]]}}}
\newcommand{\mrem}[1]{{{\small\bf [[{#1} --marco]]}}}

\newcommand{\uc}[1]{\textsc{uc}(#1)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Macros regarding the proof
%%\newcommand{\DOSMP}[1]{\textsc{do}\ensuremath{_\textsc{SYN}}(#1)\xspace}
\newcommand{\DOSMP}[1]{\textsc{do}_{\textsc{norm}}(#1)}
\newcommand{\mfSmp}[1]{\Upsilon_{#1,\textsc{norm}}}
\newcommand{\applySmp}[1]{\textsc{apply}_{\textsc{norm}}(#1)}
\newcommand{\Smp}{_{\textsc{norm}}}

\newcommand{\norm}[1]{\hat{#1}}

\newcommand{\queryeq}{\ensuremath{q^{=}}\xspace}
\newcommand{\aboxeq}{\ensuremath{A_{=}}\xspace}
\newcommand{\apply}[1]{\textsc{apply}(#1)\xspace}
%\newcommand{\applySyn}[1]{\textsc{apply}\ensuremath{_\textsc{SYN}}(#1)\xspace}
% \newcommand{\conservativeTS}{conservatice}

\newcommand{\Dummy}{\mathit{Dummy}}
\newcommand{\alphabet}[1]{\textsc{alph}(#1)}
\renewcommand{\Eq}[2][\T]{\textsc{eq}(#1,#2)}
\newcommand{\Aneq}[1]{{#1}^{\not\textsc{eq}}}

%% Turing Machine reduction

\newcommand{\tm}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\dumsym}{\texttt{\#}}
\newcommand{\ktm}{\ensuremath{\K_\tm}\xspace}
\newcommand{\blank}{\textvisiblespace}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:

